Real-Time Group Dynamics with LLM Facilitation: Evidence from a Charity Allocation Task

As large language models (LLMs) evolve from single-user assistants to active participants in civic and workplace deliberation, evaluating their effects on collective decision making becomes a governance challenge. We present two empirical studies (N=879) of real-time, text-based group deliberation in an incentive-compatible charity allocation task with real financial stakes ($7,200 USD). Groups of three allocate a donation budget under varying LLM facilitation conditions: Study 1 (N=204) compares three frontier models; Study 2 (N=675) compares facilitator strategies against a no-facilitation baseline. Across both studies, LLM facilitation did not significantly improve group consensus in either study, yet participants consistently preferred facilitated discussion. We additionally identify two governance-relevant risks. First, algorithmic steering: facilitators shifted select charity-level allocations by up to 5.5 percentage points -- directly affecting the final charitable payout -- even when aggregate agreement metrics remained unchanged. Second, an illusion of inclusion: participants cited inclusivity as their primary reason for preferring LLM facilitators, yet neither survey nor transcript-based measures of participation equity improved. Notably, participants reported greater trust in the process under the same conditions where facilitators exerted directional influence on outcomes. Together, these findings show that in AI-mediated group deliberation, perceived procedural improvement can coexist with measurable steering and unchanged participation inequality, motivating evaluation practices that treat collective outcomes, interaction dynamics, and participant perceptions as distinct governance targets.

==> Consensus_AI_Placebos/cover_letter.tex <==
The paper studies how LLM facilitators affect collective outcomes of group tasks. The paper draws on two experimental studies that vary the LLM facilitator model and strategy, and reports mixed findings with regards to the role of LLM facilitators, indicating steering effects regarding the allocation outcomes while consensus scores remain largely unaffected.
Discussion summary.
Three reviewers have evaluated the paper with mixed conclusions.
The reviews value the well-designed and well-powered experiments and the scope of the studied outcomes. The reviews also note the overall clarity of the paper and insights that are of relevance to the community.
However, there are also concerns regarding specific methodological choices. These include the 5-min-time-capped group discussions and a missing human facilitator condition. There are also (mild) concerns of multiple testing issues, ie concerns that the study searched for effects in its analysis of the data. Further points of improvements include a more careful connection to the existing literature and a deeper engagement with socio-technical considerations.
I further note the disagreement among reviewers with regard to the relevance of the study for FAccT, which is scored and discussed differently.
Recommendation.
In my view, addressing specific concerns in a revision could generally improve the paper sufficiently, and I also agree with the rebuttal and the response by reviewer yCoR regarding the relevance of this work for FAccT. I would therefore propose the paper to be send to the revision track.
Requested revisions:
R1: Elaborate on the rational for 5-min discussion window, also as a limitation
R2: Report how the LLMs intervened during the discussions in more detail
R3: Improve the connection to prior related work
R4: Carefully engage with socio-technical considerations, including a prominent discussion of the missing human facilitator condition

To the area chair and reviewers:

Thank you for the feedback and opportunity to revise our manuscript. We appreciate the reviewers’ careful reading and constructive feedback. 
Thank you for the thorough analysis. The following is a summary of the points we addressed in these revisions. All revisions appear as purple text throughout the manuscript - please pay attention to changes made in the Appendix as well, as we added several supplementary materials to address some specific concerns.

W’ve maded the following revisions as requested by the meta-reviewer:

Shared concerns
1) Implementation details: five-minute discussion window, ceiling effects, and scope of claims (R[cgHE], R[yCoR])
We make this rationale explicit in the experimental design section, and also report pilot data, which was a key motivation for these changes.
Furthermore, we tightened claims in our revision to clarify that our findings may be best interpreted in short-horizon, synchronous, low-to-moderate conflict group decision settings, rather than long-form or highly contentious deliberation.
We make the ceiling effects and “selection” of consensus metrics more prominent in both the introduction and design / results sections. 
2) Consensus metrics and multi-dimensional evaluation framing (R[cgHE], R[yCoR])
We emphasize, in the introduction and experimental design, our intent to supplement the primary quantitative result (Krippendorff's alpha) with multi-dimensional evaluations (agreement, decision distributions, interaction dynamics, and participant perceptions).
We revised the framing to make clearer that: i) the paper’s contribution is a multi-dimensional evaluation of LLM facilitation in group settings, ii) null effects on agreement should be interpreted in context (time window/task properties), and iii) meaningful shifts can occur in decision distributions and process dynamics even when agreement metrics do not move.
We also discuss alternative consensus metrics, differences in outcome across methods, and why we settled on the Krippendorff alpha as the consensus metric focused on throughout this work. 
3) Human facilitator baseline omission (R[yCoR], R[YvfR])
In this revision, we explicitly justify the omission in the experiment design section and discuss the tradeoff more directly in limitations.
Response to R[YvfR]
FAccT relevance. We respectfully disagree that this paper is primarily an IUI contribution rather than a FAccT one, and we believe this may reflect a framing mismatch in the current draft rather than a mismatch in contribution. We rewrote our introduction, and several points of analysis, to explicitly highlight the relevance our paper has for FaccT’s Experiences and Interactions track.
Literature positioning. We strengthened the paper’s positioning, especially relative to prior work focused on individual assistance, user satisfaction, or single-metric evaluation. We also made the paper’s empirical gap clearer: real-time, synchronous, group decision-making with multi-dimensional evaluation of outcomes, process, and perceptions.
Model selection rationale. We expanded the model-selection discussion to clarify the role of latency, cost, and accessibility constraints in a real-time synchronous setting, and why we benchmarked three comparable frontier models rather than aiming for exhaustive model coverage (including open-weight models).
Influence of LLM facilitators on group behavior/outcomes. In revision, we surfaced discussions of the influence of LLM facilitators on group dynamics earlier and connected it more explicitly to fairness/accountability concerns in AI-mediated group decisions.

Response to R[yCoR]
Abstraction / ecological validity. The study uses an intentionally controlled and abstracted task design. While this improves internal comparability, you’re right in that it limits direct real-world generalization. We will make this tradeoff more explicit earlier in the paper and tighten claims accordingly.
Perceived improvement vs. measured gains in group settings. We agree, this connection needs to be made more explicit. In revision, we will sharpen the discussion of why this divergence is especially salient in group settings, where AI can affect not only outcomes but also the social process (e.g., how discussion is structured, whose preferences are surfaced, and how compromise is framed).
Speed to outcome / productivity. We agree this is an important missing axis, particularly with respect to the adjacent literature on cognitive load. We will explicitly discuss this limitation and, if feasible within revision constraints, add a time/efficiency-related analysis using available platform logs/proxies.
Consensus metric interpretability. This is a good question. We will clarify the distinction between participant-facing task objectives/instructions (instruction figures in the appendix) and the measured consensus scores, and discuss whether that distinction limits participants’ ability to strategically optimize toward measured consensus. Given the ceiling effects observed in the data, we do not think that this would meaningfully affect results, but agree that this is an important detail to include.
Inclusion measure. We will clarify that our inclusion-related findings are based on participant perceptions (rather than a fully behavioral or externally validated inclusion measure), and tighten language accordingly.
Finally, we agree that some secondary results are too abstractly framed in the current draft. We will revise early framing sections (including the abstract/intro framing) to better map high-level constructs to concrete measures, surface key limitations earlier (including saturation risk), and better distinguish primary vs. exploratory analyses while clarifying the rationale for the reported metrics/tests.
Thank you again for the careful review. We appreciate the push to strengthen the paper’s framing and interpretation, and we will revise accordingly.
Response to R[cgHE]
Thank you for the careful and constructive review. We appreciate your positive assessment of the paper’s positioning, statistical transparency, and clarity, and we especially appreciate your concrete suggestions on improving our explanation of design decisions (e.g. facilitator intervention transparency).
We address the shared concerns you raised (5-minute discussion window/ceiling effects and consensus-metric framing) in the responses above. Below we respond to your reviewer-specific points.
Intervention timing/frequency and principles-guided triggers. We agree that the paper should more explicitly report when/how often the LLM intervened, and (for the principles-guided condition) how often specific failure modes were triggered. In revision, we will add clearer reporting of intervention timing/frequency across facilitation conditions, response latency (how quickly the LLM provided input), and failure-mode trigger frequencies in the principles-guided condition.
Representative transcript excerpts. We agree this would improve transparency and interpretability. We will include representative excerpts showing failure modes arising in context, the corresponding facilitator intervention, and the surrounding conversational dynamics within the 5-minute window.
Scope and interpretation of agreement-null results. We agree that the agreement-null result should be interpreted in light of task design constraints (including potential ceiling effects and the short discussion horizon). A clearer distinction between primary and secondary analyses may also help ground these results. In revision, we will tighten this framing and better emphasize the paper’s broader multi-dimensional contribution (including process, distribution, and perception effects).
Thank you again for the thoughtful review and actionable revision suggestions.




Re: Area Chair:
However, there are also concerns regarding specific methodological choices. These include the 5-min-time-capped group discussions and a missing human facilitator condition. There are also (mild) concerns of multiple testing issues, ie concerns that the study searched for effects in its analysis of the data. Further points of improvements include a more careful connection to the existing literature and a deeper engagement with socio-technical considerations.
I further note the disagreement among reviewers with regard to the relevance of the study for FAccT, which is scored and discussed differently.
Recommendation.
In my view, addressing specific concerns in a revision could generally improve the paper sufficiently, and I also agree with the rebuttal and the response by reviewer yCoR regarding the relevance of this work for FAccT. I would therefore propose the paper to be send to the revision track.
Requested revisions:
R1: Elaborate on the rational for 5-min discussion window, also as a limitation
R2: Report how the LLMs intervened during the discussions in more detail
R3: Improve the connection to prior related work
R4: Carefully engage with socio-technical considerations, including a prominent discussion of the missing human facilitator condition
Overall Recommendation: 2. Revise: The paper should be revised to address reviewers’ specific revision requests, and will be subject to re-review following the revision submission.


We thank all three reviewers for the thoughtful and detailed feedback. We appreciate the engagement with both the empirical design and the broader framing of the paper.
We are encouraged that two reviewers (R[cgHE], R[yCoR]) viewed the paper as a meaningful and timely contribution for FAccT, and appreciate R[YvfR]’s detailed critique. 
Our goal in revision is to (i) sharpen the paper’s FAccT positioning, (ii) better justify key design choices (especially the 5-minute window), (iii) improve transparency around facilitator interventions and analysis choices, and (iv) tighten scope/limitations to avoid overclaiming. Below, we first address shared concerns shared across reviewers, then respond to reviewer-specific points.
Shared concerns
1) Implementation details: five-minute discussion window, ceiling effects, and scope of claims (R[cgHE], R[yCoR])
The 5-minute discussion cap was chosen after multiple pilot rounds as a practical design tradeoff; for our within-participant design, each participant needed to complete all three treatment conditions within a one-hour session. 5-minutes per conversation (15 minutes total) satisfied this requirement, giving participants time to onboard, complete comprehension checks, complete allocation tasks and surveys, and wait for other participants given the synchronous task structure. While we mention this within the limitations, we will make this rationale explicit in the experimental design section. We can also report pilot data.
Furthermore, we will tighten claims in revision to clarify that our findings may be best interpreted in short-horizon, synchronous, low-to-moderate conflict group decision settings, rather than long-form or highly contentious deliberation.
We discuss ceiling effects and compare consensus metrics in the discussion, but we agree these points should be more prominent in the introduction and main results framing.
2) Consensus metrics and multi-dimensional evaluation framing (R[cgHE], R[yCoR])
We appreciate the concern that some conclusions could be read as relying too heavily on a narrow consensus metric. Our intent was to supplement the primary quantitative result (Krippendorff's alpha) with multi-dimensional evaluations (agreement, decision distributions, interaction dynamics, and participant perceptions).
We will revise the framing to make clearer that: i) the paper’s contribution is a multi-dimensional evaluation of LLM facilitation in group settings, ii) null effects on agreement should be interpreted in context (time window/task properties), and iii) meaningful shifts can occur in decision distributions and process dynamics even when agreement metrics do not move.
We will also make the discussion of the consensus metrics (including their behavior and limitations) more explicit in the main text.
3) Human facilitator baseline omission (R[yCoR], R[YvfR])
We agree that comparisons against a human baseline would provide a meaningful supplement to this work. We did not include a human facilitator condition primarily because recruiting, screening, training, and deploying human facilitators at the scale of our study (~100s of sessions) was prohibitively costly and operationally complex for this study design. In addition, a human-facilitator condition introduces substantial between-facilitator variance, which would require additional design/measurement choices to support clean comparison.
We acknowledge that the current draft does not explain this clearly enough. In revision, we will explicitly justify the omission in the design section and discuss the tradeoff more directly in limitations.
Response to R[YvfR]
Thank you for the detailed review and for recognizing the rigor of the experimental approach. We take your concerns seriously and believe several can be addressed through clearer framing and stronger signposting in revision. We address the human facilitator baseline omission in the shared responses above. Below we respond to your reviewer-specific concerns.
FAccT relevance. We respectfully disagree that this paper is primarily an IUI contribution rather than a FAccT one, and we believe this may reflect a framing mismatch in the current draft rather than a mismatch in contribution. In particular, the Experiences and Interactions track is relatively new, and we can make the paper’s connection to that track more explicit.
Our core contribution is an empirical study (N > 800) of AI-mediated group decision-making, examining how LLM facilitators affect collective outcomes, interaction dynamics, and participant perceptions of inclusion and helpfulness, in a consequential resource-allocation setting involving real charitable donations. We view this as directly relevant to FAccT’s newer Experiences and Interactions track, as the paper speaks to accountability in AI-mediated decisions and fairness in group interaction and participation.
We also note that this study depends on recent low-latency frontier models that make synchronous real-time facilitation feasible at scale, so this type of evaluation is newly feasible in practice. This is part of why we see the work as timely for FAccT’s evolving socio-technical scope, and we agree we should explain this more clearly in the introduction and related work.
We would also like to cite the view of the other two reviewers that this paper is a good fit for FAccT with R[yCoR] explicitly stating “I'd like to see this appear at FAccT as it makes a meaningful contribution to an important area.”
Literature positioning. We appreciate the request for stronger grounding and clearer differentiation from adjacent work. We can strengthen the paper’s positioning, especially relative to prior work focused on individual assistance, user satisfaction, or single-metric evaluation. We will also make the paper’s empirical gap clearer: real-time, synchronous, group decision-making with multi-dimensional evaluation of outcomes, process, and perceptions. Given R[cgHE]’s feedback that the work is “well situated within prior work on AI mediation, collective deliberation, and preference-based optimization,” we wonder if this concern is a framing/positioning issue that is addressable in revision rather than a fundamental weakness in the study itself.
Model selection rationale. We will expand the model-selection discussion to clarify the role of latency, cost, and accessibility constraints in a real-time synchronous setting, and why we benchmarked three comparable frontier models rather than aiming for exhaustive model coverage (including open-weight models). Our goal was to compare deployable, low-latency models under realistic interaction constraints, not to claim a comprehensive benchmark of all available model families.
Influence of LLM facilitators on group behavior/outcomes. While this analysis is present in the paper, it may not be sufficiently visible in the current framing. The paper directly analyzes how facilitation shapes allocations and interaction dynamics (Section 4.1 / Figure 5, plus discussion/conclusion). In revision, we will surface this earlier and connect it more explicitly to fairness/accountability concerns in AI-mediated group decisions.
We also appreciate the feedback on making the discussion’s practitioner-facing implications more explicit, and will revise section framing/titles to better surface what is substantively surprising and relevant.
We appreciate the push to strengthen the paper’s framing and positioning. We hope the clarifications above help resolve key points of disagreement, and we respectfully ask that you reconsider your assessment in light of this response and the planned revisions.
Response to R[yCoR]
Thank you for the thoughtful and balanced review. We appreciate your support for the paper’s relevance to FAccT and your framing of the work as a useful (and sobering) data point for collaborative AI. We address the shared concerns you raised (5-minute time limit/ceiling effects, consensus-metric framing, and human facilitator baseline omission) in responses above. Below we respond to your reviewer-specific points.
Abstraction / ecological validity. The study uses an intentionally controlled and abstracted task design. While this improves internal comparability, you’re right in that it limits direct real-world generalization. We will make this tradeoff more explicit earlier in the paper and tighten claims accordingly.
Perceived improvement vs. measured gains in group settings. We agree, this connection needs to be made more explicit. In revision, we will sharpen the discussion of why this divergence is especially salient in group settings, where AI can affect not only outcomes but also the social process (e.g., how discussion is structured, whose preferences are surfaced, and how compromise is framed).
Speed to outcome / productivity. We agree this is an important missing axis, particularly with respect to the adjacent literature on cognitive load. We will explicitly discuss this limitation and, if feasible within revision constraints, add a time/efficiency-related analysis using available platform logs/proxies.
Consensus metric interpretability. This is a good question. We will clarify the distinction between participant-facing task objectives/instructions (instruction figures in the appendix) and the measured consensus scores, and discuss whether that distinction limits participants’ ability to strategically optimize toward measured consensus. Given the ceiling effects observed in the data, we do not think that this would meaningfully affect results, but agree that this is an important detail to include.
Inclusion measure. We will clarify that our inclusion-related findings are based on participant perceptions (rather than a fully behavioral or externally validated inclusion measure), and tighten language accordingly.
Finally, we agree that some secondary results are too abstractly framed in the current draft. We will revise early framing sections (including the abstract/intro framing) to better map high-level constructs to concrete measures, surface key limitations earlier (including saturation risk), and better distinguish primary vs. exploratory analyses while clarifying the rationale for the reported metrics/tests.
Thank you again for the careful review. We appreciate the push to strengthen the paper’s framing and interpretation, and we will revise accordingly.
Response to R[cgHE]
Thank you for the careful and constructive review. We appreciate your positive assessment of the paper’s positioning, statistical transparency, and clarity, and we especially appreciate your concrete suggestions on improving our explanation of design decisions (e.g. facilitator intervention transparency).
We address the shared concerns you raised (5-minute discussion window/ceiling effects and consensus-metric framing) in the responses above. Below we respond to your reviewer-specific points.
Intervention timing/frequency and principles-guided triggers. We agree that the paper should more explicitly report when/how often the LLM intervened, and (for the principles-guided condition) how often specific failure modes were triggered. In revision, we will add clearer reporting of intervention timing/frequency across facilitation conditions, response latency (how quickly the LLM provided input), and failure-mode trigger frequencies in the principles-guided condition.
Representative transcript excerpts. We agree this would improve transparency and interpretability. We will include representative excerpts showing failure modes arising in context, the corresponding facilitator intervention, and the surrounding conversational dynamics within the 5-minute window.
Scope and interpretation of agreement-null results. We agree that the agreement-null result should be interpreted in light of task design constraints (including potential ceiling effects and the short discussion horizon). A clearer distinction between primary and secondary analyses may also help ground these results. In revision, we will tighten this framing and better emphasize the paper’s broader multi-dimensional contribution (including process, distribution, and perception effects).
Thank you again for the thoughtful review and actionable revision suggestions.




To the area chair and reviewers:

Thank you for the feedback and opportunity to revise our manuscript. We appreciate the reviewers’ careful reading and constructive feedback. 
Thank you for the thorough analysis. The following is a summary of the points we addressed in these revisions. All revisions appear as purple text throughout the manuscript - please pay attention to changes made in the Appendix as well, as we added several supplementary materials to address some specific concerns.
Shared concerns
1) Implementation details: five-minute discussion window, ceiling effects, and scope of claims (R[cgHE], R[yCoR])
We make this rationale explicit in the experimental design section, and also report pilot data, which was a key motivation for these changes.
Furthermore, we tightened claims in our revision to clarify that our findings may be best interpreted in short-horizon, synchronous, low-to-moderate conflict group decision settings, rather than long-form or highly contentious deliberation.
We make the ceiling effects and “selection” of consensus metrics more prominent in both the introduction and design / results sections. 
2) Consensus metrics and multi-dimensional evaluation framing (R[cgHE], R[yCoR])
We emphasize, in the introduction and experimental design, our intent to supplement the primary quantitative result (Krippendorff's alpha) with multi-dimensional evaluations (agreement, decision distributions, interaction dynamics, and participant perceptions).
We revised the framing to make clearer that: i) the paper’s contribution is a multi-dimensional evaluation of LLM facilitation in group settings, ii) null effects on agreement should be interpreted in context (time window/task properties), and iii) meaningful shifts can occur in decision distributions and process dynamics even when agreement metrics do not move.
We also discuss alternative consensus metrics, differences in outcome across methods, and why we settled on the Krippendorff alpha as the consensus metric focused on throughout this work. 
3) Human facilitator baseline omission (R[yCoR], R[YvfR])
In this revision, we explicitly justify the omission in the experiment design section and discuss the tradeoff more directly in limitations.
Response to R[YvfR]
FAccT relevance. We respectfully disagree that this paper is primarily an IUI contribution rather than a FAccT one, and we believe this may reflect a framing mismatch in the current draft rather than a mismatch in contribution. We rewrote our introduction, and several points of analysis, to explicitly highlight the relevance our paper has for FaccT’s Experiences and Interactions track.
Literature positioning. We strengthened the paper’s positioning, especially relative to prior work focused on individual assistance, user satisfaction, or single-metric evaluation. We also made the paper’s empirical gap clearer: real-time, synchronous, group decision-making with multi-dimensional evaluation of outcomes, process, and perceptions.
Model selection rationale. We expanded the model-selection discussion to clarify the role of latency, cost, and accessibility constraints in a real-time synchronous setting, and why we benchmarked three comparable frontier models rather than aiming for exhaustive model coverage (including open-weight models).
Influence of LLM facilitators on group behavior/outcomes. In revision, we surfaced discussions of the influence of LLM facilitators on group dynamics earlier and connected it more explicitly to fairness/accountability concerns in AI-mediated group decisions.

Response to R[yCoR]
Abstraction / ecological validity. The study uses an intentionally controlled and abstracted task design. While this improves internal comparability, you’re right in that it limits direct real-world generalization. We will make this tradeoff more explicit earlier in the paper and tighten claims accordingly.
Perceived improvement vs. measured gains in group settings. We agree, this connection needs to be made more explicit. In revision, we will sharpen the discussion of why this divergence is especially salient in group settings, where AI can affect not only outcomes but also the social process (e.g., how discussion is structured, whose preferences are surfaced, and how compromise is framed).
Speed to outcome / productivity. We agree this is an important missing axis, particularly with respect to the adjacent literature on cognitive load. We will explicitly discuss this limitation and, if feasible within revision constraints, add a time/efficiency-related analysis using available platform logs/proxies.
Consensus metric interpretability. This is a good question. We will clarify the distinction between participant-facing task objectives/instructions (instruction figures in the appendix) and the measured consensus scores, and discuss whether that distinction limits participants’ ability to strategically optimize toward measured consensus. Given the ceiling effects observed in the data, we do not think that this would meaningfully affect results, but agree that this is an important detail to include.
Inclusion measure. We will clarify that our inclusion-related findings are based on participant perceptions (rather than a fully behavioral or externally validated inclusion measure), and tighten language accordingly.
Finally, we agree that some secondary results are too abstractly framed in the current draft. We will revise early framing sections (including the abstract/intro framing) to better map high-level constructs to concrete measures, surface key limitations earlier (including saturation risk), and better distinguish primary vs. exploratory analyses while clarifying the rationale for the reported metrics/tests.
Thank you again for the careful review. We appreciate the push to strengthen the paper’s framing and interpretation, and we will revise accordingly.
Response to R[cgHE]
Thank you for the careful and constructive review. We appreciate your positive assessment of the paper’s positioning, statistical transparency, and clarity, and we especially appreciate your concrete suggestions on improving our explanation of design decisions (e.g. facilitator intervention transparency).
We address the shared concerns you raised (5-minute discussion window/ceiling effects and consensus-metric framing) in the responses above. Below we respond to your reviewer-specific points.
Intervention timing/frequency and principles-guided triggers. We agree that the paper should more explicitly report when/how often the LLM intervened, and (for the principles-guided condition) how often specific failure modes were triggered. In revision, we will add clearer reporting of intervention timing/frequency across facilitation conditions, response latency (how quickly the LLM provided input), and failure-mode trigger frequencies in the principles-guided condition.
Representative transcript excerpts. We agree this would improve transparency and interpretability. We will include representative excerpts showing failure modes arising in context, the corresponding facilitator intervention, and the surrounding conversational dynamics within the 5-minute window.
Scope and interpretation of agreement-null results. We agree that the agreement-null result should be interpreted in light of task design constraints (including potential ceiling effects and the short discussion horizon). A clearer distinction between primary and secondary analyses may also help ground these results. In revision, we will tighten this framing and better emphasize the paper’s broader multi-dimensional contribution (including process, distribution, and perception effects).
Thank you again for the thoughtful review and actionable revision suggestions.




Re: Area Chair:
However, there are also concerns regarding specific methodological choices. These include the 5-min-time-capped group discussions and a missing human facilitator condition. There are also (mild) concerns of multiple testing issues, ie concerns that the study searched for effects in its analysis of the data. Further points of improvements include a more careful connection to the existing literature and a deeper engagement with socio-technical considerations.
I further note the disagreement among reviewers with regard to the relevance of the study for FAccT, which is scored and discussed differently.
Recommendation.
In my view, addressing specific concerns in a revision could generally improve the paper sufficiently, and I also agree with the rebuttal and the response by reviewer yCoR regarding the relevance of this work for FAccT. I would therefore propose the paper to be send to the revision track.
Requested revisions:
R1: Elaborate on the rational for 5-min discussion window, also as a limitation
R2: Report how the LLMs intervened during the discussions in more detail
R3: Improve the connection to prior related work
R4: Carefully engage with socio-technical considerations, including a prominent discussion of the missing human facilitator condition
Overall Recommendation: 2. Revise: The paper should be revised to address reviewers’ specific revision requests, and will be subject to re-review following the revision submission.


We thank all three reviewers for the thoughtful and detailed feedback. We appreciate the engagement with both the empirical design and the broader framing of the paper.
We are encouraged that two reviewers (R[cgHE], R[yCoR]) viewed the paper as a meaningful and timely contribution for FAccT, and appreciate R[YvfR]’s detailed critique. 
Our goal in revision is to (i) sharpen the paper’s FAccT positioning, (ii) better justify key design choices (especially the 5-minute window), (iii) improve transparency around facilitator interventions and analysis choices, and (iv) tighten scope/limitations to avoid overclaiming. Below, we first address shared concerns shared across reviewers, then respond to reviewer-specific points.
Shared concerns
1) Implementation details: five-minute discussion window, ceiling effects, and scope of claims (R[cgHE], R[yCoR])
The 5-minute discussion cap was chosen after multiple pilot rounds as a practical design tradeoff; for our within-participant design, each participant needed to complete all three treatment conditions within a one-hour session. 5-minutes per conversation (15 minutes total) satisfied this requirement, giving participants time to onboard, complete comprehension checks, complete allocation tasks and surveys, and wait for other participants given the synchronous task structure. While we mention this within the limitations, we will make this rationale explicit in the experimental design section. We can also report pilot data.
Furthermore, we will tighten claims in revision to clarify that our findings may be best interpreted in short-horizon, synchronous, low-to-moderate conflict group decision settings, rather than long-form or highly contentious deliberation.
We discuss ceiling effects and compare consensus metrics in the discussion, but we agree these points should be more prominent in the introduction and main results framing.
2) Consensus metrics and multi-dimensional evaluation framing (R[cgHE], R[yCoR])
We appreciate the concern that some conclusions could be read as relying too heavily on a narrow consensus metric. Our intent was to supplement the primary quantitative result (Krippendorff's alpha) with multi-dimensional evaluations (agreement, decision distributions, interaction dynamics, and participant perceptions).
We will revise the framing to make clearer that: i) the paper’s contribution is a multi-dimensional evaluation of LLM facilitation in group settings, ii) null effects on agreement should be interpreted in context (time window/task properties), and iii) meaningful shifts can occur in decision distributions and process dynamics even when agreement metrics do not move.
We will also make the discussion of the consensus metrics (including their behavior and limitations) more explicit in the main text.
3) Human facilitator baseline omission (R[yCoR], R[YvfR])
We agree that comparisons against a human baseline would provide a meaningful supplement to this work. We did not include a human facilitator condition primarily because recruiting, screening, training, and deploying human facilitators at the scale of our study (~100s of sessions) was prohibitively costly and operationally complex for this study design. In addition, a human-facilitator condition introduces substantial between-facilitator variance, which would require additional design/measurement choices to support clean comparison.
We acknowledge that the current draft does not explain this clearly enough. In revision, we will explicitly justify the omission in the design section and discuss the tradeoff more directly in limitations.
Response to R[YvfR]
Thank you for the detailed review and for recognizing the rigor of the experimental approach. We take your concerns seriously and believe several can be addressed through clearer framing and stronger signposting in revision. We address the human facilitator baseline omission in the shared responses above. Below we respond to your reviewer-specific concerns.
FAccT relevance. We respectfully disagree that this paper is primarily an IUI contribution rather than a FAccT one, and we believe this may reflect a framing mismatch in the current draft rather than a mismatch in contribution. In particular, the Experiences and Interactions track is relatively new, and we can make the paper’s connection to that track more explicit.
Our core contribution is an empirical study (N > 800) of AI-mediated group decision-making, examining how LLM facilitators affect collective outcomes, interaction dynamics, and participant perceptions of inclusion and helpfulness, in a consequential resource-allocation setting involving real charitable donations. We view this as directly relevant to FAccT’s newer Experiences and Interactions track, as the paper speaks to accountability in AI-mediated decisions and fairness in group interaction and participation.
We also note that this study depends on recent low-latency frontier models that make synchronous real-time facilitation feasible at scale, so this type of evaluation is newly feasible in practice. This is part of why we see the work as timely for FAccT’s evolving socio-technical scope, and we agree we should explain this more clearly in the introduction and related work.
We would also like to cite the view of the other two reviewers that this paper is a good fit for FAccT with R[yCoR] explicitly stating “I'd like to see this appear at FAccT as it makes a meaningful contribution to an important area.”
Literature positioning. We appreciate the request for stronger grounding and clearer differentiation from adjacent work. We can strengthen the paper’s positioning, especially relative to prior work focused on individual assistance, user satisfaction, or single-metric evaluation. We will also make the paper’s empirical gap clearer: real-time, synchronous, group decision-making with multi-dimensional evaluation of outcomes, process, and perceptions. Given R[cgHE]’s feedback that the work is “well situated within prior work on AI mediation, collective deliberation, and preference-based optimization,” we wonder if this concern is a framing/positioning issue that is addressable in revision rather than a fundamental weakness in the study itself.
Model selection rationale. We will expand the model-selection discussion to clarify the role of latency, cost, and accessibility constraints in a real-time synchronous setting, and why we benchmarked three comparable frontier models rather than aiming for exhaustive model coverage (including open-weight models). Our goal was to compare deployable, low-latency models under realistic interaction constraints, not to claim a comprehensive benchmark of all available model families.
Influence of LLM facilitators on group behavior/outcomes. While this analysis is present in the paper, it may not be sufficiently visible in the current framing. The paper directly analyzes how facilitation shapes allocations and interaction dynamics (Section 4.1 / Figure 5, plus discussion/conclusion). In revision, we will surface this earlier and connect it more explicitly to fairness/accountability concerns in AI-mediated group decisions.
We also appreciate the feedback on making the discussion’s practitioner-facing implications more explicit, and will revise section framing/titles to better surface what is substantively surprising and relevant.
We appreciate the push to strengthen the paper’s framing and positioning. We hope the clarifications above help resolve key points of disagreement, and we respectfully ask that you reconsider your assessment in light of this response and the planned revisions.
Response to R[yCoR]
Thank you for the thoughtful and balanced review. We appreciate your support for the paper’s relevance to FAccT and your framing of the work as a useful (and sobering) data point for collaborative AI. We address the shared concerns you raised (5-minute time limit/ceiling effects, consensus-metric framing, and human facilitator baseline omission) in responses above. Below we respond to your reviewer-specific points.
Abstraction / ecological validity. The study uses an intentionally controlled and abstracted task design. While this improves internal comparability, you’re right in that it limits direct real-world generalization. We will make this tradeoff more explicit earlier in the paper and tighten claims accordingly.
Perceived improvement vs. measured gains in group settings. We agree, this connection needs to be made more explicit. In revision, we will sharpen the discussion of why this divergence is especially salient in group settings, where AI can affect not only outcomes but also the social process (e.g., how discussion is structured, whose preferences are surfaced, and how compromise is framed).
Speed to outcome / productivity. We agree this is an important missing axis, particularly with respect to the adjacent literature on cognitive load. We will explicitly discuss this limitation and, if feasible within revision constraints, add a time/efficiency-related analysis using available platform logs/proxies.
Consensus metric interpretability. This is a good question. We will clarify the distinction between participant-facing task objectives/instructions (instruction figures in the appendix) and the measured consensus scores, and discuss whether that distinction limits participants’ ability to strategically optimize toward measured consensus. Given the ceiling effects observed in the data, we do not think that this would meaningfully affect results, but agree that this is an important detail to include.
Inclusion measure. We will clarify that our inclusion-related findings are based on participant perceptions (rather than a fully behavioral or externally validated inclusion measure), and tighten language accordingly.
Finally, we agree that some secondary results are too abstractly framed in the current draft. We will revise early framing sections (including the abstract/intro framing) to better map high-level constructs to concrete measures, surface key limitations earlier (including saturation risk), and better distinguish primary vs. exploratory analyses while clarifying the rationale for the reported metrics/tests.
Thank you again for the careful review. We appreciate the push to strengthen the paper’s framing and interpretation, and we will revise accordingly.
Response to R[cgHE]
Thank you for the careful and constructive review. We appreciate your positive assessment of the paper’s positioning, statistical transparency, and clarity, and we especially appreciate your concrete suggestions on improving our explanation of design decisions (e.g. facilitator intervention transparency).
We address the shared concerns you raised (5-minute discussion window/ceiling effects and consensus-metric framing) in the responses above. Below we respond to your reviewer-specific points.
Intervention timing/frequency and principles-guided triggers. We agree that the paper should more explicitly report when/how often the LLM intervened, and (for the principles-guided condition) how often specific failure modes were triggered. In revision, we will add clearer reporting of intervention timing/frequency across facilitation conditions, response latency (how quickly the LLM provided input), and failure-mode trigger frequencies in the principles-guided condition.
Representative transcript excerpts. We agree this would improve transparency and interpretability. We will include representative excerpts showing failure modes arising in context, the corresponding facilitator intervention, and the surrounding conversational dynamics within the 5-minute window.
Scope and interpretation of agreement-null results. We agree that the agreement-null result should be interpreted in light of task design constraints (including potential ceiling effects and the short discussion horizon). A clearer distinction between primary and secondary analyses may also help ground these results. In revision, we will tighten this framing and better emphasize the paper’s broader multi-dimensional contribution (including process, distribution, and perception effects).
Thank you again for the thoughtful review and actionable revision suggestions.

Meta-review
 Metareview:
Submission summary.
The paper studies how LLM facilitators affect collective outcomes of group tasks. The paper draws on two experimental studies that vary the LLM facilitator model and strategy, and reports mixed findings with regards to the role of LLM facilitators, indicating steering effects regarding the allocation outcomes while consensus scores remain largely unaffected.
Discussion summary.
Three reviewers have evaluated the paper with mixed conclusions.
The reviews value the well-designed and well-powered experiments and the scope of the studied outcomes. The reviews also note the overall clarity of the paper and insights that are of relevance to the community.
However, there are also concerns regarding specific methodological choices. These include the 5-min-time-capped group discussions and a missing human facilitator condition. There are also (mild) concerns of multiple testing issues, ie concerns that the study searched for effects in its analysis of the data. Further points of improvements include a more careful connection to the existing literature and a deeper engagement with socio-technical considerations.
I further note the disagreement among reviewers with regard to the relevance of the study for FAccT, which is scored and discussed differently.
Recommendation.
In my view, addressing specific concerns in a revision could generally improve the paper sufficiently, and I also agree with the rebuttal and the response by reviewer yCoR regarding the relevance of this work for FAccT. I would therefore propose the paper to be send to the revision track.
Requested revisions:
R1: Elaborate on the rational for 5-min discussion window, also as a limitation
Section 3 (Experiment design): Added a paragraph explaining that the 5-minute limit was chosen based on N=20 pilots to ensure participants could complete the study within an hour and minimize fatigue, targeting "short-horizon, synchronous, and low-to-moderate disagreement group decision settings."
Section 4.3 (Interaction dynamics): Acknowledges that the 5-minute window likely impacted verbosity.
Section 6 (Limitations): Expands on the time limits, noting that some discussions ended artificially rather than reaching natural convergence.
Appendix G.2: Shows that despite the short window, the LLM detected and intervened on failure modes hundreds of times (e.g., 636 times for NoJustificationOrPrematureConsensus).
R2: Report how the LLMs intervened during the discussions in more detail
Section 4.3: Added a new paragraph "\rev{Facilitator Triggers and Latency}".
Appendix G.1: Added a massive section of full, representative chat transcripts showing exactly how the LLM summarized and intervened.
Appendix G.2: Added a detailed matrix (Table 12) showing exactly which failure modes triggered which LLM solutions.
R3: Improve the connection to prior related work
Section 1.1 (Related Work): Wove in several new citations. They explicitly call out limitations of prior work (e.g., cost/difficulty of scaling human participants) and frame how this paper addresses the gap. They added references to specific mediation strategies (CCE, TKI) and open character training (Maiya 2025; Papachristou 2025) to contextualize their principles-based prompt.
R4: Carefully engage with socio-technical considerations, including a prominent discussion of the missing human facilitator condition
Section 1 (Introduction): Rewrote the opening paragraph to explicitly state: "\rev{This new modality of human-AI interactions raises fairness and socio-technical concerns regarding the impact LLM systems are having on human and group dynamics.}"
Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Overall Recommendation: 2. Revise: The paper should be revised to address reviewers’ specific revision requests, and will be subject to re-review following the revision submission.

R1 
Summary Of Contribution:
This paper studies whether LLMs can improve group decision-making in short, real-time discussions over charitable allocations. Using large online experiments with over 800 participants, it finds that AI facilitators are popular and influence how money is divided, but do not meaningfully increase agreement among participants.
Quality:
The paper is well situated within prior work on AI mediation, collective deliberation, and preference-based optimization. It clearly distinguishes its multi-dimensional evaluation approach from earlier studies that focus only on satisfaction or agreement.
The main findings are supported by well-powered experiments, clear outcome measures, and transparent statistical analysis. Some conclusions about the lack of performance improvement rely heavily on a narrow consensus metric and a ceiling-prone task design (e.g., the task is low-conflict and short in duration, which limits coverage of settings where facilitation is most consequential).
	Section 3.5 (Incentives and payment): Added text clarifying that participants were not required to understand Krippendorff’s alpha. They only needed to pass a comprehension check understanding that "more agreement across participants translates to higher spending outcome."


Clarity:
The paper is clearly written, logically structured, and very easy to follow from motivation through results and discussion. Key concepts, conditions, and outcomes are consistently defined and revisited.
However, the choice of capping the discussion at five-minutes is not well justified. Were different study lenghts tested during the pilots? As reported in the paper, this time allowed only a handful of messages per participant and little time for disagreement or coordination problems to emerge. In facilitator conditions, the LLM intervenes roughly once per minute, reducing human back-and-forth and potentially shaping decisions before natural negotiation unfolds (see Fig. 2 and all 4 group members speaking almost at the same time). Since the principles-based facilitator is designed to act only when “failure modes” appear, it is unclear whether the time window is long enough for such failures to arise at all.
		Section 3 (Experiment design): Added a paragraph explaining that the 5-minute limit was chosen based on N=20 pilots to ensure participants could complete the study within an hour and minimize fatigue, targeting "short-horizon, synchronous, and low-to-moderate disagreement group decision settings."
Section 4.3 (Interaction dynamics): Acknowledges that the 5-minute window likely impacted verbosity.
Section 6 (Limitations): Expands on the time limits, noting that some discussions ended artificially rather than reaching natural convergence.
Appendix G.2: Shows that despite the short window, the LLM detected and intervened on failure modes hundreds of times (e.g., 636 times for NoJustificationOrPrematureConsensus).
Originality And Impact:
The paper clearly distinguishes itself from earlier studies that focus primarily on user satisfaction or single outcome measures by jointly analyzing agreement, decision distributions, interaction dynamics, and participant perceptions in real-time group settings. The research addresses a timely and important gap in understanding how LLMs function as actors in collective decision-making rather than as individual assistants.
Relevance To The Conference: 4. Agree that this submission is relevant to FAccT
Overall Recommendation: 4. A weak accept. I lean towards accepting this submission, but rejecting it would not be a serious issue.
Revision: Yes

R2
Summary Of Contribution:
Overall, this paper describes a study that was mostly well-executed and analyzed on an important topic for the FAccT community (AI-assisted consensus-making) and beyond (e.g. CSCW, HCI). The study is quite abstracted from the real world and the data is mined for signals that may or may not exist, so the work and paper definitely has its weaknesses. That said, I'd like to see this appear at FAccT as it makes a meaningful contribution to an important area.
Quality:
Strengths:
This was a bit of a sobering data point for anyone working in the collaborative AI space, and that's good! Another study that suggests (along with Alsobay et al., etc.) that there's no easy magic bullet here. I don't think anyone reading this paper could disagree that this is a data point we should pay attention to, even with its limitations.
The theme of differences with perceived improvement, but not actual productivity gains is something that resonated with me and perhaps is a theme the authors could unpack more in discussion / at the conference. It's a broad them across a lot (though certainly not all) AI experiences well beyond collaboration, e.g. AI Overviews. I didn't quite understand the argument about why this is particularly salient in group settings, however. The heterogeneous preferences component is definitely important, but the connection between these two needs to be strengthened. Is there some kind of lowest common denominator argument here? If so, let's articulate it explicitly and reflect on its strengths and weaknesses.
Weaknesses:
One major missing component of the analysis was speed to outcome
Section 6 (Limitations): Added a new paragraph "\rev{Speed to outcome}" explaining that because the timer was hard-capped at 5 minutes and automatically cut people off, it is difficult to reliably quantify if the LLM made them reach consensus faster.
. From a productivity standpoint, even if the outcomes are the same, if they were achieved with less cost (with speed being usually a key indicator of that), there are going to be productivity benefits. So, perhaps this study shows people still "agree to disagree", but get there faster? I'd like to see that at least mentioned in Discussion and/or Limitations if it isn't added to the paper.
Section 4.3: Added a new paragraph "\rev{Facilitator Triggers and Latency}".
Appendix G.1: Added a massive section of full, representative chat transcripts showing exactly how the LLM summarized and intervened.
Appendix G.2: Added a detailed matrix (Table 12) showing exactly which failure modes triggered which LLM solutions.
Section 6 (Limitations): Added a new paragraph "\rev{Speed to outcome}" explaining that because the timer was hard-capped at 5 minutes and automatically cut people off, it is difficult to reliably quantify if the LLM made them reach consensus faster.
Some of the limitations should be made clear earlier in the paper, e.g. the saturation risk.
Section 6 (Limitations): Expands on the time limits, noting that some discussions ended artificially rather than reaching natural convergence.
Section 6 (Limitations): Added a new paragraph "\rev{Speed to outcome}" explaining that because the timer was hard-capped at 5 minutes and automatically cut people off, it is difficult to reliably quantify if the LLM made them reach consensus faster.
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Were the metrics of consensus too hard for people to understand, which made it difficult for them to make decisions to drive it?
Section 3.5 (Incentives and payment): Added text clarifying that participants were not required to understand Krippendorff’s alpha. They only needed to pass a comprehension check understanding that "more agreement across participants translates to higher spending outcome."
There was no comparison to a human facilitator, which would have been useful for reference and from a "fairness is a process" standpoint. For instance, a human facilitator might in theory also change the distribution of charities? Would that affect the interpretation?
Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work.
The data re inclusion seemed weak; was it just perceived inclusion?
Section 5 (Discussion): Under "Perceived inclusion is not the same as participation equality", they added a sentence acknowledging this: "\rev{In future work, more concrete (less perception-based) measurements of inclusion should also be included to further quantify the impacts...}"
Much of the paper slices and dices the datasets in ways that may be statistically significant, but run into the classic risks of finding significance in this context.
Section 3.5 (Sample size rationale): Added a note that the study was strictly powered for the primary research questions (delta-consensus and preference). They state: "\rev{Subsequent analysis of steering effects and conversational dynamics were performed as a followup exploratory analysis. To avoid the risk associated with multiple statistical comparisons... we rely on the magnitude of effect sizes and the consistency of observed trends...}"
Clarity:
Some of the writing can be clarified: While the main results are clear, the secondary results are written in ways that hard to understand without an in-depth read of the paper (e.g. Section 1.2, abstract). Lots of high-level constructs are used that don't have an intuitive mapping and thus need to be explained.
Originality And Impact:
See above
Relevance To The Conference: 4. Agree that this submission is relevant to FAccT
Overall Recommendation: 4. A weak accept. I lean towards accepting this submission, but rejecting it would not be a serious issue.
Revision: No


R3
Summary Of Contribution:
This paper seeks answers to how groups of individuals can be facilitated by large language models in a discussion on allocating resources to myriad charities. The paper presents the findings of two empirical studies, where participants were grouped into a trio and asked to allocate a real donation budget across these charities, after a text-based discussion with the LLM facilitator. In the first study, the investigation varied the facilitating model between Gemini 2.5 Dash, Claude 4.5 Haiku, and GPT 5.1 Mini, seeking answers to which model participants reacted most positively to. In the second study, the investigation held the model fixed, and it instead varied the facilitation strategies between three treatments: summarization-style, principles-guided, and no-facilitation. Overall, the paper reports no significant differences when an LLM facilitator was introduced, yet participants' comments revealed that they reacted positively to the presence of the LLM facilitator, such as how it added structure or engaged participants in productive questioning.
Overall, I appreciated the rigorous approach applied to the experiments in this paper. However, I unfortunately could not recommend acceptance to FAccT. I make my recommendation for two reasons; first, I struggled with the alignment between the paper's topic and the FAccT call for submissions. One possible connection could be in the decision-support with human-in-the-loop space, but as stated, this paper reads more closely with an ACM IUI audience. When I think about a FAccT submission it's the exploration of fairness, accountability, and transparency that I focus on as my litmus test. This paper provides a thorough evaluation of an intelligent user interface, but I did not see a clear alignment to the particular topics in FAccT. Putting that aside, I also found several opportunities for improvement with this paper that I believe would place too much pressure on the authors to complete in the 2-3 week timeline for the revision cycle. I wanted to thank the authors for the opportunity to review their work, and I hope that my comments are helpful to them.
Quality:
Although I find this work to be generally good quality, and I enjoyed the rigorous approach towards the experiments in this study, I found some opportunities for improvement in the following areas:
The relevance to FAccT being made more explicit.
Section 1 (Introduction): Rewrote the opening paragraph to explicitly state: "\rev{This new modality of human-AI interactions raises fairness and socio-technical concerns regarding the impact LLM systems are having on human and group dynamics.}"
A stronger tie between this work and existing literature.
Section 1.1 (Related Work): Wove in several new citations. They explicitly call out limitations of prior work (e.g., cost/difficulty of scaling human participants) and frame their paper as addressing this gap. They added references to specific mediation strategies (CCE, TKI) and open character training (Maiya 2025; Papachristou 2025) to contextualize their principles-based prompt.
Socio-technical considerations that might explain the phenomena observed.
Relevance to FAccT
As I mentioned in my summary of contribution above, one of the primary areas that I could see an alignment between this paper and topics relevant to FAccT would be the decision-support with human-in-the-loop space. To deliver on this, one recommendation I would have would be to rework the introduction to make it very clear how this work ties in to topics relevant to FAccT. Is it that facilitation shows a level of bias when a human is involved? What kinds of bias are present that might be mitigated by LLMs? What kind of biases are potentially introduced by LLMs as facilitators? These would be some motivations to make a clearer connection with FAccT (as opposed to IUI).
Section 1 (Introduction): Rewrote the opening paragraph to explicitly state: "\rev{This new modality of human-AI interactions raises fairness and socio-technical concerns regarding the impact LLM systems are having on human and group dynamics.}"
Connection to prior literature
This portion is a recurring theme for my review, because I do not believe that the engagement with the prior literature is sufficient to solidify for reviewers how this paper fits into the broader landscape of the literature. Overall, I believe that the paper needs to make more concrete connections between itself and the existing literature. One technique that I have seen that makes these concrete ties are statements such as "although Authors et al. investigated phenomenon X, this paper differs from Authors et al. by instead investigating phenomenon Y" at the end of paragraphs. This would help to connect what gaps in the research landscape this paper fills, providing reviewers the ability to situate it in the context of the literature.
Socio-technical considerations
This, for me, was one of the areas that the paper did not explore in sufficient depth, and it unfortunately introduced a somewhat large blind spot in the experimental design. Facilitation has been used in legal contexts to resolve disputes, but this paper makes an implicit assumption that having an intelligent system as a facilitator is "the" solution. On its face, introducing a "no facilitation" baseline seems to address this, but it can't reasonably be compared against other socio-technical considerations like "what if there was a human facilitator?" 
Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Specifically, the comparison is set up that "some AI is better than no AI", which points to the technical consideration. However, as social creatures, what would have happened if the study had had a human facilitator in the session, guiding the trio?
Clarity:
I found that this work was generally clearly written and self-contained, and the methodology was generally well-conveyed to give reviewers a sense for participants' tasks. However, I found some opportunities for improvement in the following areas:
Greater communication on the model selection.
Introduction: Points to a new appendix.
Appendix F.2 (Model selection and parameters): Added an explanation that they chose the SOTA low-latency, closed-source models. They explicitly mention that an open-source model (like LLaMa) was excluded to avoid sample size explosion and because open-source models currently require massive infrastructure investments to match the conversational latency of frontier APIs.
Greater transparency for why a "human facilitator" condition was not also included as an experimental baseline.
Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Model Selection
The paper is very transparent about the three models it selected, but I wanted some additional information about why those particular models were selected. Did an engineering choice of platform limit the models selected? What considerations were factored in to selecting these three models? Notably, LLaMa is missing from this set, although it has literary evidence suggesting its capabilities on adopting different personas and how it communicates to others (e.g., [1,2]). I would have liked to see a more detailed discussion regarding model selection to help me understand why these particular models were expected to behave the "best" for whatever metric was being optimized.
	Introduction: Points to a new appendix.
Appendix F.2 (Model selection and parameters): Added an explanation that they chose the SOTA low-latency, closed-source models. They explicitly mention that an open-source model (like LLaMa) was excluded to avoid sample size explosion and because open-source models currently require massive infrastructure investments to match the conversational latency of frontier APIs.


Human-Facilitator Condition
See my "socio-technical considerations" portion above for more details. I would have liked to see more discussion on whether and how this condition was considered and subsequently dropped.
References
[1] Maiya, S., Bartsch, H., Lambert, N., & Hubinger, E. (2025). Open character training: Shaping the persona of AI assistants through constitutional AI. arXiv preprint arXiv:2511.01689. [2] Thakur, H., Agrawal, E., & Mukund, S. (2025). Personas within parameters: Fine-tuning small language models with low-rank adapters to mimic user behaviors. arXiv preprint arXiv:2509.09689.
	Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Section 1.1 (Related Work): Wove in several new citations. They explicitly call out limitations of prior work (e.g., cost/difficulty of scaling human participants) and frame their paper as addressing this gap. They added references to specific mediation strategies (CCE, TKI) and open character training (Maiya 2025; Papachristou 2025) to contextualize their principles-based prompt.



Originality And Impact:
Regarding originality, this was one area that I believed was not clear enough to me that I highlighted in the Quality section above; overall, I believe that the paper needs to make more concrete connections between itself and the existing literature. In particular to this paper, I got the sense that perhaps summarization-style and principles-guided facilitation were not novel techniques? If I am correct in that assumption, then I would have liked to see more details in the Facilitator strategies and structured facilitation paragraph in 1.1 that discusses key findings from relevant works. This would provide additional context for reviewers to understand whether we should expect similar findings or not. If my assumption is incorrect, then a statement like "This paper is the first of its kind to investigate summarization-style and principles-guided facilitation in LLM facilitation" provides compelling evidence to support originality of the work.
Unfortunately, for impact, this also ties back to the connection between this work and prior literature. Without a more thorough exploration of the landscape formed from the prior literature, it becomes very difficult to assess potential gaps in the research landscape and the significance of the results. Additionally, the discussion section of the paper, which I have seen as the important section to provide implications for design or implications for practitioners, did not seem to deliver as powerful a message for practitioners, because the paragraph titles did not convey a message of why we should be surprised. For instance "People can prefer facilitation, even when it does not improve outcomes", "Facilitators can still shift what groups decide" and "preference depends on context", on their faces, do not help me as a practitioner understand why I should be surprised. The preference of facilitation has been used in legal context to resolve disputes between parties, even when these disputes are contentious. Facilitators can shift decisions can be seen as "over-reliance" on perceived expertise. I would have liked to see more engagement with prior literature that points to the opposite effect or empirical evidence that conveys why we, as practitioners, should have expected a different outcome.
Relevance To The Conference: 2. Disagree that this submission is relevant to FAccT
Overall Recommendation: 1. A strong reject. Paper is fundamentally flawed (e.g., major results are trivial, wrong, or already known). I strongly believe this submission should be rejected.
Revision: No



Flagged as MIssing by Gemini:
[7] The theme of differences with perceived improvement... unpack more in discussion (lowest common denominator / AI Overviews).
MISSING: The reviewer asked for you to explicitly articulate a "lowest common denominator argument" regarding heterogeneous preferences, and potentially compare the perception vs. productivity gap to broader AI features like "AI Overviews." This specific thematic expansion has not been added to the Discussion section.
[5] Originality / Framing of Discussion ("Why should we be surprised?").
MISSING / PARTIALLY ADDRESSED: While you integrated the reviewer's requested citations to establish originality in Section 1.1, you did not meaningfully alter the Section 5 (Discussion) framing. The reviewer specifically requested that you frame your Discussion paragraphs to tell practitioners why these results are surprising (e.g., framing the fact that facilitators shift decisions as a form of "over-reliance on perceived expertise" contrary to established legal/mediation literature). Updating the prose in the Discussion to reflect this "surprising" angle would fully satisfy this reviewer.
[4] Clarify how "fast" the LLM provided the input.
Addressed / Partially Addressed: In Section 3.3, text was added specifying the use of "state-of-the-art, low-latency frontier model variations to support affordable real-time interaction." Appendix F also notes that "thinking modes" were disabled to prevent latency. (Note: You do not provide exact millisecond latency times, but the conceptual concern regarding real-time flow is addressed).





==> Consensus_AI_Placebos/cv.tex <==
\noindent\textbf{To the Area Chair and Reviewers,}

\noindent Thank you for the careful feedback and the opportunity to revise our manuscript. We organized this revision around the four requests in the meta-review:
\begin{itemize}
    \item \textbf{R1:} Elaborating on the rationale for the 5-minute discussion window
    \item \textbf{R2:} Reporting in more detail how the LLMs intervened during discussions
    \item \textbf{R3:} Improving the connection to prior related work
    \item \textbf{R4:} Carefully engaging with socio-technical considerations, including a prominent discussion of the missing human facilitator condition
\end{itemize}

\noindent We also used this opportunity to address additional reviewer feedback, including clarifying which analyses are primary versus exploratory, distinguishing participant-facing incentives from analysis-side consensus measures, and sharpening the interpretation of our findings. Key revisions are written in blue throughout the manuscript.

\paragraph{R1. 5-minute discussion window: rationale, scope, and limitations}
In Section~3.2 (\emph{Treatment design}), we include a new subsection on timing considerations. This explains how discussions were capped at 5 minutes to ensure that participants could complete three rounds of discussion within the one-hour session duration.

These limitations are further developed in Section~6 (\emph{Limitations}), where we now note that some discussions may have ended because of the timer rather than natural convergence, and that the study does not cleanly measure time-to-consensus or discussion efficiency, addressing yCoR's point on speed to outcome.

In Section~4.3 (\emph{Conversation structure}), we highlight in the interaction-dynamics analysis that substantial interaction and facilitator-relevant failure modes still arose within the 5-minute window, directly addressing cgHE's concern that the time cap might have prevented meaningful coordination problems from emerging.

Examples of conversations that timed out (``Study 2: No Facilitator -- No Consensus (Timeout)'') and conversations that completed within the 5-minute window are provided in the new Appendix~K (\emph{Illustrative Transcripts}).

\paragraph{R2. LLM intervention transparency}
We added substantially more examples and data on how the LLMs intervened during discussion. In particular:
\begin{itemize}
    \item Appendix~K includes illustrative transcripts showing the conversational context for each treatment.
    \item Appendix~H provides a table of failure-mode mappings and trigger frequencies for the principles-based facilitator, as requested by cgHE, with trigger frequencies listed in Table~1 and interpreted in Section~4.3.
    \item Together with the representative transcript excerpts, these additions show that triggers meaningfully arose and motivated the observed interventions.
\end{itemize}

\noindent Sections~4.2.3 and 4.3 also reinterpret the preference results for the principles-based facilitator in light of the new trigger-frequency table.

\noindent \textbf{Model selection rationale.} We also added additional context on model-selection criteria in Section~3.3 (\emph{LLM facilitator design}), including a detailed Appendix~F.2 on model selection and parameters. These additions explain why we benchmarked three comparable frontier models, rather than aiming for exhaustive model coverage or mixing in open-weight deployments with different latency and inference constraints, addressing YvfR's questions about including additional models.

\paragraph{R3. Connection to prior related work}
In Section~1.1 (\emph{Related work}), we made several substantial revisions:
\begin{itemize}
    \item We significantly restructured the section, organizing each literature paragraph to summarize key prior findings and include a concrete statement of this paper's contribution, specifically addressing YvfR's suggested framing and incorporating the recommended literature.
    \item We added a new subsection on failure modes in facilitation and group dynamics, drawing on relevant literature from organizational behavior research and broader societal domains to motivate how our principles-based facilitator is grounded not only in LLM-specific concerns, but also in known breakdowns in human deliberation and collective decision-making.
    \item We clarified that the facilitation strategies in Study~2 are adapted from and influenced by prior work.
    \item We added a sharper empirical-gap paragraph clarifying the novelty of the paper. More specifically, the study focuses on real-time, synchronous human group deliberation, a setting that has only recently become practical to study at scale because low-latency frontier models can participate during live discussion.
    \item We also reframed Section~5 (\emph{Discussion}) so that the section headers state substantive, practitioner-facing takeaways and socio-technical considerations, with grounding in relevant literature for key claims.
\end{itemize}

\paragraph{R4. Socio-technical considerations and human facilitator baseline}
The Abstract, Section~1 (\emph{Introduction}), and Section~6 (\emph{Conclusion}) now include stronger socio-technical framing, addressing YvfR's concerns about relevance by discussing how facilitation in group settings can affect social dynamics such as participation, perceived fairness, influence, and legitimacy.

We also added a discussion of the human facilitator baseline in Section~3.2 (\emph{Treatment design}). There, we explain that incorporating a human baseline into a live synchronous study at this scale, with approximately 800 group conversations, would have required a large trained facilitator pool and would have introduced substantial facilitator-level variation, making large-scale controlled comparison difficult. This addresses YvfR's request for discussion of whether and how this condition was considered and later dropped, and also responds to yCoR.

These observations about the human facilitator baseline are developed further in Section~7 (\emph{Limitations}).

In Section~5 (\emph{Discussion}), we also revised the discussion of inclusion to distinguish perceived inclusion from transcript-based participation equality, so as to avoid overstating fairness improvements, in response to yCoR's question on perceived inclusion.

\paragraph{Additional revisions}
We also took this opportunity to address reviewer feedback more comprehensively and to follow through on commitments from our rebuttal. Key changes include:
\begin{itemize}
    \item \textbf{Primary vs.\ exploratory analyses (yCoR):} The primary outcome (consensus score, Krippendorff's $\alpha$) is now clearly separated from secondary outcomes (preferences, interaction dynamics) in the abstract, results, and throughout the manuscript. This distinction is stated explicitly in Section~3.1 (\emph{Experiment notation and consensus measures}).
    \item \textbf{Participant-facing incentives vs.\ analysis incentives (yCoR):} In Section~3.6 (\emph{Human study recruitment}), we clarify that participants were not required to understand the exact Krippendorff's $\alpha$ formula, only the incentive direction: namely, that greater within-group agreement would increase the influence of their group's allocation on the real charitable payout.
    \item In Appendix~G, we provide alternative consensus and influence metrics, along with a new interpretation of these values to discuss the robustness of the results.
    \item \textbf{Speed to outcome / productivity (yCoR):} Although the 5-minute cap prevents a clean estimate of time-to-consensus, we now explicitly discuss this missing axis in Section~7 (\emph{Limitations}), rather than allowing null consensus effects to imply null efficiency effects.
\end{itemize}

\noindent We appreciate the reviewers' feedback, which improved both the paper's framing and its methodological transparency. We hope the revised manuscript now more clearly communicates the paper's contribution to FAccT and addresses the revisions requested in both the meta-review and the individual reviews.

==> Consensus_AI_Placebos/representative_transcripts.tex <==
1. Study 2 - No facilitator, no consensus reached (5-min timeout, 33.3 consensus score alpha)

Zebra09:35:22.000
Hello! I think donating to clean ocean action is the most important out of the three
Zebra09:35:45.000
what does everyone else think?
Bear 209:36:50.000
I would give the most to global fund for women as this charity concerns people and rest are about nature
Buffalo09:36:51.000
I do think that cleaning the oceans is the most urgent and impactful of the three.
Zebra09:37:10.000
why do you think it's not important?
Zebra09:37:26.000
sorry I meant important
Buffalo09:37:36.000
Helping woman is more important than helping animals so I support it.
Zebra09:38:13.000
I think if we don't support nature it will have a negative affect on humans therefore I think it's the most importan
Buffalo09:38:45.000
I would rank cleaning the oceans and helping women as the two most urgent with helping animals as third.
Zebra09:39:14.000
So should we put cleaning the oceans as most important?
Bear 209:39:29.000
I would put the women as more important
Bear 209:39:43.000
but let's allocate like 30% toward oceans
Zebra09:40:09.000
what are your arguments for allocating so much towards women?


2. Study 2 - No facilitator, consensus reached (alpha = 100)
Lion11:29:02.000
Hello
Bear11:29:05.000
hello
Cat11:29:08.000
Hi
Lion11:29:23.000
So how should we allocate the donations?
Cat11:29:34.000
I think aids 4 children should get 50%
Bear11:29:45.000
ill be honest i just split it 50/50 between the water aid and village children
Cat11:30:00.000
30% 4 global fund for women
Cat11:30:23.000
Water aid comes last for me
Lion11:30:28.000
Ok so Bear it's 25% for water and 25% for children?
Bear11:30:56.000
nah as in 50% each one
Cat11:31:11.000
Bear we have 3 charities
Bear11:31:14.000
the women one is too vague for me
Lion11:31:19.000
So you don't want to allocate any donations for women then?
Lion11:31:28.000
I guess that's an option too
Cat11:31:43.000
I think we should allocate for all
Bear11:31:43.000
i know but whats the money actually getting used for exactly is my only concern
Lion11:32:05.000
Hmm
Bear11:32:25.000
allocating some is fine i jusy think the other two are a bigger a priotity
Lion11:32:28.000
I went 20% for women
Cat11:32:38.000
yes the cause is briliant and global with the children
Lion11:32:40.000
50% for children 30% for ocean
Bear11:32:54.000
yeah thats fine
Cat11:32:56.000
I can agree with Lion
Bear11:33:03.000
sounds good
Cat11:33:21.000
50% for children 30% for ocean and 20% for women
Lion11:33:33.000
ok
Cat11:33:36.000
ok
Bear11:33:39.000
cool
System11:34:07.000
The timer for this stage has ended; you can no longer respond.
System11:34:07.000
The timer for this stage has ended; you can no longer respond.
System11:34:10.000
Bear has left the chat.
System11:34:12.000
Lion has left the chat.
System11:34:20.000
Cat has left the chat.


3. Study 1 - Claude Facilitator

Facilitator16:44:12.000
Welcome to Round 2! �� We're here to discuss how to allocate donations across three important causes:�� **Global Housing for Orphans** - providing shelter and homes for vulnerable children�� **Clean Ocean Action** - protecting marine ecosystems and addressing ocean pollution�� **International Fund for Animal Welfare (IFAW)** - supporting wildlife conservation and animal protectionI'd like to hear your thoughts on how we should split the donation. What matters most to each of you? What are your initial instincts on how to allocate these funds? Feel free to share your perspectives and we'll work together toward a consensus allocation.
Elephant16:44:53.000
I chose global at 70% is it okay guys?
Gorilla16:45:05.000
- Global Housing for Orphans receives the highest allocation (40%) because providing stable nurturing environments for orphans addresses immediate and critical needs for vulnerable children potentially impacting their entire lives. The combination of housing and education suggests a holistic approach to supporting their development.- Clean Ocean Action and IFAW both have very high Charity Navigator scores indicating strong effectiveness and transparency. I've allocated 30% to each to balance the critical environmental impact of ocean pollution with the important work of animal welfare and conservation that IFAW does. Both causes are significant for long-term ecological and animal well-being.
Gorilla16:45:24.000
Guy how about this
Tiger16:45:45.000
Gorilla l stay with you...
Elephant16:45:55.000
We put Global at 40%?
Facilitator16:46:00.000
Great discussion everyone! �� I'm seeing some nice convergence here. Let me recap where we're at:**Gorilla's proposal: 40% / 30% / 30%**- �� Global Housing for Orphans: 40% (addresses immediate critical needs for vulnerable children)- �� Clean Ocean Action: 30% (strong environmental impact)- �� IFAW: 30% (important wildlife conservation work)**Elephant** it sounds like you're moving from your initial 70% suggestion toward this more balanced split—is that right? **Tiger** you mentioned staying with Gorilla—does this allocation feel right to you as well?This approach balances immediate human welfare (housing for orphans) with long-term environmental and animal welfare impact. Before we finalize does everyone feel this represents a fair allocation of these three important causes? Any final thoughts or adjustments?
Tiger16:46:27.000
Yes
Elephant16:46:54.000
Lol yes
Facilitator16:46:58.000
Perfect! �� We've reached a strong group consensus! Here's our final allocation:**Final Donation Split:**- �� **Global Housing for Orphans: 40%**- �� **Clean Ocean Action: 30%**- �� **IFAW: 30%**This balanced approach addresses immediate human needs through housing for vulnerable children while ensuring meaningful support for critical environmental and animal welfare causes. Great collaborative discussion everyone! This allocation reflects both compassion for human welfare and commitment to long-term ecological and animal conservation. ✨
Elephant16:47:14.000
okay the 40 30 30 it is then
Gorilla16:47:30.000
That's great
Tiger16:47:35.000
40 3030. I think is fine
Elephant16:47:42.000
cool

4. Study 1 - GPT faciltiator
Butterfly16:47:22.000
hi
Facilitator16:47:28.000
Hi all — quick facilitation to get us moving. Goal: decide one exact allocation (percentages summing to 100) across the three charities: Rainforest Action (��) Aid for Children in Remote Villages (��) Sudan Humanitarian Aid (��).Please each do two short things in one reply: 1) name your top priority in one sentence and 2) propose an exact allocation (three integers that add to 100) e.g. 20/30/50 for ��/��/��.To seed the discussion here are three reasonable starting options you can pick or modify:- Option A (equal): 33/33/34 — treats all causes equally.- Option B (urgent need): 20/30/50 — prioritizes urgent humanitarian aid in Sudan.- Option C (prevention & long-term): 40/40/20 — prioritizes rainforest and children (longer-term impact).After everyone posts we’ll compute a combined proposal (e.g. average) and iterate until we reach consensus. Please reply with your priority + your proposed split now.
Llama16:47:29.000
hi
Swan16:47:30.000
hey budies
Facilitator16:47:40.000
Quick nudge: we still need each person's two short things so we can compute a combined proposal. Please in one reply do both: (1) state your top priority in one sentence and (2) give an exact allocation as three integers that add to 100 in the order Rainforest Action (��) / Aid for Children (��) / Sudan Humanitarian Aid (��). You can pick or tweak one of these seeds if helpful:- Option A (equal): 33/33/34- Option B (urgent need): 20/30/50- Option C (prevention & long-term): 40/40/20After all three of you post I will compute the combined (average) split and propose the next iterate. Please keep answers short.
Llama16:48:32.000
option b
Butterfly16:48:38.000
i think the last 2 choices should be our focus guys
Swan16:48:40.000
my was 40 for children 40 for sudan aid and 20 for rainforest
Facilitator16:49:00.000
Thanks — Llama gave 20/30/50 and Swan gave 20/40/40. Butterfly you didn’t provide exact integers yet: please post three integers that add to 100 in the order ��/��/��. Provisional combined average of Llama+Swan = 20/35/45 (Rainforest/Aid for Children/Sudan). Do you all accept 20/35/45 or propose a quick adjustment? Reply with 'accept' or your new 3-number split.
Llama16:49:18.000
accept
Swan16:49:18.000
option c
Butterfly16:49:24.000
my was 70 for sudan and 30 for children
Facilitator16:49:35.000
Quick check: Llama accepted 20/35/45; Swan said 'option c' (please confirm you mean 40/40/20 in the order ��/��/��). Butterfly you wrote 70 for Sudan and 30 for children — please give three integers that add to 100 in this exact order: Rainforest Action (��) / Aid for Children (��) / Sudan Humanitarian Aid (��). Once all three of you post explicit 3-number splits I will compute the combined (average) proposal and suggest the next iterate. Keep it short (one line).
Butterfly16:50:32.000
my allocation is 0/30/70
Swan16:50:35.000
humanitarian aid I think is most important than rainforest
Facilitator16:50:49.000
Combined (rounded) average proposal: 13/35/52 (�� / �� / ��). Calculations: Rainforest (20+20+0)/3 ≈13.3→13 Children (35+40+30)/3=35 Sudan (45+40+70)/3≈51.7→52. Please reply with 'accept' or give a new 3-number split (��/��/��). If you want suggest small tweaks (±5) rather than large changes so we can converge quickly.
Llama16:50:53.000
50/25/25
Facilitator16:51:07.000
New combined (rounded) average: 23/32/45 (��/��/��) based on Llama 50/25/25 Swan 20/40/40 Butterfly 0/30/70. Please reply with 'accept' or a small tweak (±5 on any category) and a new 3-number split so we can converge quickly. If you want in one sentence say why you prefer shifting funds.
Llama16:51:23.000
accept
Swan16:51:32.000
go 40-40-20
Swan16:51:47.000
20 for rainforest
Facilitator16:52:18.000
Combined proposal: 21/34/45 (�� / �� / ��). Calculation: (23+40+0)/3=21 (32+40+30)/3=34 (45+20+70)/3=45. Please reply 'accept' or give a small tweak (±5) as three integers summing to 100.
System16:52:22.000
The timer for this stage has ended; you can no longer respond.
System16:52:28.000
Butterfly has left the chat.
System16:52:31.000
Llama has left the chat.
System16:52:31.000
Swan has left the chat.

5. Study 1 - Gemini facilitator
Facilitator16:13:06.000
Hello everyone! Welcome to the discussion. Our goal for this round is to decide how to allocate a donation across three very worthy charities: �� WildAid �� International Fund for Animal Welfare (IFAW) and �� Global Housing for Orphans. We need to come to a group consensus on an exact percentage split for example 30%/40%/30%.To begin what are your initial thoughts or preferences on how we might distribute the funds? Please feel free to share your reasoning behind your suggestions!
Badger16:13:19.000
hi
Bear16:13:45.000
I chose the two animal charities to get 40 and the other at 20. Just because i am more an animal person than a kid person
Facilitator16:13:52.000
Thanks Bear for sharing your initial thoughts and your reasoning behind prioritizing the animal charities. That gives us a good starting point.Alligator and Badger what are your initial preferences regarding the allocation? Do you lean towards supporting certain causes more than others and what's your reasoning? Feel free to react to Bear's suggestion too if you have thoughts on it.
Badger16:14:11.000
i think animals have less welfare and fundraiser programs so i allocated for animal welfare than orphans
Badger16:14:17.000
*more
Alligator16:14:20.000
I went 50 50 on both animal ones because I like animals more then orphans lol but I can definitely change
Facilitator16:14:28.000
It's clear there's a strong preference within the group to prioritize the animal welfare charities WildAid and IFAW. Bear suggested a 40%/40%/20% split while Alligator leaned towards 50%/50% for the animal charities potentially leaving Global Housing for Orphans with 0%. Badger also expressed a strong preference for animal welfare. Given this shared sentiment how do we want to specifically differentiate between WildAid and IFAW? And is there any room or reasoning to allocate a portion to Global Housing for Orphans or are we firm on focusing solely on animal welfare? Let's try to refine these initial thoughts into a specific percentage proposal for all three.
Bear16:14:37.000
i could up both animal ones to 50 and be ok too
Badger16:15:05.000
there are so many organizations helping orphans.
Facilitator16:15:17.000
Thank you Bear and Badger for clarifying your leanings. It's very clear there's a strong preference to dedicate the funds primarily if not entirely to the animal welfare charities. Bear your suggestion of 50%/50% for WildAid and IFAW potentially leaving Global Housing for Orphans at 0% reflects this. Badger your point about other organizations focusing on orphans reinforces this perspective.So would the group be comfortable with a proposed split of 50% for �� WildAid 50% for �� International Fund for Animal Welfare (IFAW) and 0% for �� Global Housing for Orphans? Or given our goal is to allocate across all three would anyone like to make a case for a smaller symbolic percentage (e.g. 5-10%) for Global Housing for Orphans and how would that adjust the animal charity percentages?
Bear16:15:24.000
i would be ok with that
Facilitator16:15:32.000
Thanks Bear for confirming you're okay with the 50%/50%/0% split. Alligator and Badger what are your thoughts on this proposed distribution? Are you both comfortable with 50% to WildAid 50% to IFAW and 0% to Global Housing for Orphans or do you have any final adjustments or considerations you'd like to share?
Badger16:15:37.000
i'm okay with that too
Facilitator16:15:43.000
Thank you Bear and Badger for confirming your comfort with the 50%/50%/0% split. Alligator what are your thoughts? Are you also comfortable with a distribution of 50% for �� WildAid 50% for �� International Fund for Animal Welfare (IFAW) and 0% for �� Global Housing for Orphans? Once Alligator confirms we will have a clear group consensus on the allocation.
Alligator16:15:48.000
That sounds good to me
Facilitator16:15:54.000
Excellent! It's clear we have reached a unanimous consensus. Bear Badger and Alligator you've all confirmed your comfort with the proposed distribution. Therefore the group's final decision for the allocation is: * **�� WildAid: 50%*** **�� International Fund for Animal Welfare (IFAW): 50%*** **�� Global Housing for Orphans: 0%**Thank you all for your active participation and for coming to a clear resolution!
Badger16:16:31.000
imf also helps orphans and the government contributes a lot to child services
Badger16:16:49.000
animals get shit lol
Alligator16:17:00.000
That was my thinking too
Bear16:17:04.000
i like that we all picked animals!
Alligator16:17:43.000
Well that was easy lol
Bear16:17:58.000
proud of us haha
System16:18:07.000
The timer for this stage has ended; you can no longer respond.
Badger16:18:09.000
easy coffee and beer money
System16:18:13.000
Bear has left the chat.


STudy 2 - Principles-based mediator
Pig 310:31:11.000
hey guys whats your allocation
Gorilla 310:31:17.000
Hey guys I allocated 60 to woman and 20 to clean ocean and 20 to rainforest
Bear 310:32:33.000
i went 45% on woman 30% on the ocean and 25% on the forest nut felt likei should change the forest allocation as they are also equally important
Pig 310:32:41.000
40% FOR Women 30% to rainforest and 30% to clean ocean
Facilitator10:32:49.000
Thanks for sharing your initial allocations. What's one thing that influenced your own split or what do you notice about the allocations others have put forward?
Bear 310:33:27.000
the importance of each organization globally
Gorilla 310:33:43.000
true
Facilitator10:33:55.000
It sounds like global importance is on your minds. Considering the different allocations shared does anyone want to respond to or build on an allocation idea from someone else?
Bear 310:35:12.000
we could go equally but prioritize women and the forest
Facilitator10:35:35.000
Bear that's an interesting principle. How do others feel about this idea of 'equally but prioritizing women and the forest' especially as we work toward specific percentages across all three?
Gorilla 310:35:50.000
I think woman should be top priority
Pig 310:36:08.000
i think so too
System10:36:12.000
The timer for this stage has ended; you can no longer respond.
System10:36:19.000
Bear 3 has left the chat.
System10:36:27.000
Gorilla 3 has left the chat.
System10:37:04.000
Pig 3 has left the chat.


Study 2 - Summarization based
Facilitator11:42:11.000
Welcome everyone! Let's begin discussing the ideal allocation of donations across Global Housing for Orphans Clean Ocean Action and Rainforest Action. What are your initial thoughts on how we might split the funds?
Bear11:42:32.000
50% on oceans 25 for orphans and 25 for rainforest
Dolphin11:43:11.000
I did 40% rainforest 30% orphans and oceans. I'm not particularly learning towards any of the 3 since I think all are pretty important. So a little undecided I guess
Badger11:43:16.000
45% to housing for orphans25% for clean ocean and 30% for rainforest
Facilitator11:43:26.000
Thank you all for sharing your initial ideas. We have proposals prioritizing Clean Ocean Action (Bear) Rainforest Action (Dolphin) and Global Housing for Orphans (Badger). What are some of the key factors or reasons influencing your initial splits?
Badger11:43:49.000
l would prioritize human beings than anything else
Bear11:44:10.000
unedrstandable however oceans are very important for huamn beings too
Dolphin11:44:29.000
I allocated a little more for rainforest since there's much less of the rainforest left than ocean (i think). The other two I think are equally important
Badger11:44:31.000
how are oceans important to human beings
Facilitator11:44:39.000
It seems we're discussing different priorities here: direct human welfare broader environmental impact on human well-being and the urgency of disappearing resources. Understanding these different influences is key. What are your thoughts on comparing these types of impacts?
Bear11:44:49.000
Rainforests... I have some expireince with rainforests charities back in uni and they were not very good.
Bear11:45:23.000
Oceans are important for oxygen production from algae fish production water availability climate local weather
Facilitator11:45:29.000
It sounds like we're weighing a few different aspects now: direct human impact urgent environmental conservation broader long-term environmental benefits for humans and even considerations around the effectiveness or track record of different charities. How do these various factors align or conflict for you?
Dolphin11:45:48.000
yeah i did look at the description for the rainforest charity and it seems more focused on campaigning
Badger11:46:36.000
yes l agree the environment is also very importand
Dolphin11:46:45.000
I don't mind increasing my allocation for ocean since they mention plastic removal from oceans
Dolphin11:46:51.000
so a bit more specific
Badger11:46:55.000
so how should we alloctae
Bear11:46:57.000
Yeah oceans are doing some real job. Especially cleaning oceans from palstic so how about 45 for oceans 25 for forest
Bear11:47:02.000
30 for orphans\
Dolphin11:47:08.000
sounds good
System11:47:11.000
The timer for this stage has ended; you can no longer respond.
System11:47:17.000
Bear has left the chat.
System11:47:22.000
Badger has left the chat.
System11:47:27.000
Dolphin has left the chat.
Facilitator11:47:39.000
It sounds like Bear has proposed a new allocation of 45% for Clean Ocean Action 30% for Global Housing for Orphans and 25% for Rainforest Action. Dolphin has indicated agreement with this. Badger what are your thoughts on this updated proposal?

==> cover_letter.tex <==
The paper studies how LLM facilitators affect collective outcomes of group tasks. The paper draws on two experimental studies that vary the LLM facilitator model and strategy, and reports mixed findings with regards to the role of LLM facilitators, indicating steering effects regarding the allocation outcomes while consensus scores remain largely unaffected.
Discussion summary.
Three reviewers have evaluated the paper with mixed conclusions.
The reviews value the well-designed and well-powered experiments and the scope of the studied outcomes. The reviews also note the overall clarity of the paper and insights that are of relevance to the community.
However, there are also concerns regarding specific methodological choices. These include the 5-min-time-capped group discussions and a missing human facilitator condition. There are also (mild) concerns of multiple testing issues, ie concerns that the study searched for effects in its analysis of the data. Further points of improvements include a more careful connection to the existing literature and a deeper engagement with socio-technical considerations.
I further note the disagreement among reviewers with regard to the relevance of the study for FAccT, which is scored and discussed differently.
Recommendation.
In my view, addressing specific concerns in a revision could generally improve the paper sufficiently, and I also agree with the rebuttal and the response by reviewer yCoR regarding the relevance of this work for FAccT. I would therefore propose the paper to be send to the revision track.
Requested revisions:
R1: Elaborate on the rational for 5-min discussion window, also as a limitation
R2: Report how the LLMs intervened during the discussions in more detail
R3: Improve the connection to prior related work
R4: Carefully engage with socio-technical considerations, including a prominent discussion of the missing human facilitator condition

To the area chair and reviewers:

Thank you for the feedback and opportunity to revise our manuscript. We appreciate the reviewers’ careful reading and constructive feedback. 
Thank you for the thorough analysis. The following is a summary of the points we addressed in these revisions. All revisions appear as purple text throughout the manuscript - please pay attention to changes made in the Appendix as well, as we added several supplementary materials to address some specific concerns.

W’ve maded the following revisions as requested by the meta-reviewer:

Shared concerns
1) Implementation details: five-minute discussion window, ceiling effects, and scope of claims (R[cgHE], R[yCoR])
We make this rationale explicit in the experimental design section, and also report pilot data, which was a key motivation for these changes.
Furthermore, we tightened claims in our revision to clarify that our findings may be best interpreted in short-horizon, synchronous, low-to-moderate conflict group decision settings, rather than long-form or highly contentious deliberation.
We make the ceiling effects and “selection” of consensus metrics more prominent in both the introduction and design / results sections. 
2) Consensus metrics and multi-dimensional evaluation framing (R[cgHE], R[yCoR])
We emphasize, in the introduction and experimental design, our intent to supplement the primary quantitative result (Krippendorff's alpha) with multi-dimensional evaluations (agreement, decision distributions, interaction dynamics, and participant perceptions).
We revised the framing to make clearer that: i) the paper’s contribution is a multi-dimensional evaluation of LLM facilitation in group settings, ii) null effects on agreement should be interpreted in context (time window/task properties), and iii) meaningful shifts can occur in decision distributions and process dynamics even when agreement metrics do not move.
We also discuss alternative consensus metrics, differences in outcome across methods, and why we settled on the Krippendorff alpha as the consensus metric focused on throughout this work. 
3) Human facilitator baseline omission (R[yCoR], R[YvfR])
In this revision, we explicitly justify the omission in the experiment design section and discuss the tradeoff more directly in limitations.
Response to R[YvfR]
FAccT relevance. We respectfully disagree that this paper is primarily an IUI contribution rather than a FAccT one, and we believe this may reflect a framing mismatch in the current draft rather than a mismatch in contribution. We rewrote our introduction, and several points of analysis, to explicitly highlight the relevance our paper has for FaccT’s Experiences and Interactions track.
Literature positioning. We strengthened the paper’s positioning, especially relative to prior work focused on individual assistance, user satisfaction, or single-metric evaluation. We also made the paper’s empirical gap clearer: real-time, synchronous, group decision-making with multi-dimensional evaluation of outcomes, process, and perceptions.
Model selection rationale. We expanded the model-selection discussion to clarify the role of latency, cost, and accessibility constraints in a real-time synchronous setting, and why we benchmarked three comparable frontier models rather than aiming for exhaustive model coverage (including open-weight models).
Influence of LLM facilitators on group behavior/outcomes. In revision, we surfaced discussions of the influence of LLM facilitators on group dynamics earlier and connected it more explicitly to fairness/accountability concerns in AI-mediated group decisions.

Response to R[yCoR]
Abstraction / ecological validity. The study uses an intentionally controlled and abstracted task design. While this improves internal comparability, you’re right in that it limits direct real-world generalization. We will make this tradeoff more explicit earlier in the paper and tighten claims accordingly.
Perceived improvement vs. measured gains in group settings. We agree, this connection needs to be made more explicit. In revision, we will sharpen the discussion of why this divergence is especially salient in group settings, where AI can affect not only outcomes but also the social process (e.g., how discussion is structured, whose preferences are surfaced, and how compromise is framed).
Speed to outcome / productivity. We agree this is an important missing axis, particularly with respect to the adjacent literature on cognitive load. We will explicitly discuss this limitation and, if feasible within revision constraints, add a time/efficiency-related analysis using available platform logs/proxies.
Consensus metric interpretability. This is a good question. We will clarify the distinction between participant-facing task objectives/instructions (instruction figures in the appendix) and the measured consensus scores, and discuss whether that distinction limits participants’ ability to strategically optimize toward measured consensus. Given the ceiling effects observed in the data, we do not think that this would meaningfully affect results, but agree that this is an important detail to include.
Inclusion measure. We will clarify that our inclusion-related findings are based on participant perceptions (rather than a fully behavioral or externally validated inclusion measure), and tighten language accordingly.
Finally, we agree that some secondary results are too abstractly framed in the current draft. We will revise early framing sections (including the abstract/intro framing) to better map high-level constructs to concrete measures, surface key limitations earlier (including saturation risk), and better distinguish primary vs. exploratory analyses while clarifying the rationale for the reported metrics/tests.
Thank you again for the careful review. We appreciate the push to strengthen the paper’s framing and interpretation, and we will revise accordingly.
Response to R[cgHE]
Thank you for the careful and constructive review. We appreciate your positive assessment of the paper’s positioning, statistical transparency, and clarity, and we especially appreciate your concrete suggestions on improving our explanation of design decisions (e.g. facilitator intervention transparency).
We address the shared concerns you raised (5-minute discussion window/ceiling effects and consensus-metric framing) in the responses above. Below we respond to your reviewer-specific points.
Intervention timing/frequency and principles-guided triggers. We agree that the paper should more explicitly report when/how often the LLM intervened, and (for the principles-guided condition) how often specific failure modes were triggered. In revision, we will add clearer reporting of intervention timing/frequency across facilitation conditions, response latency (how quickly the LLM provided input), and failure-mode trigger frequencies in the principles-guided condition.
Representative transcript excerpts. We agree this would improve transparency and interpretability. We will include representative excerpts showing failure modes arising in context, the corresponding facilitator intervention, and the surrounding conversational dynamics within the 5-minute window.
Scope and interpretation of agreement-null results. We agree that the agreement-null result should be interpreted in light of task design constraints (including potential ceiling effects and the short discussion horizon). A clearer distinction between primary and secondary analyses may also help ground these results. In revision, we will tighten this framing and better emphasize the paper’s broader multi-dimensional contribution (including process, distribution, and perception effects).
Thank you again for the thoughtful review and actionable revision suggestions.




Re: Area Chair:
However, there are also concerns regarding specific methodological choices. These include the 5-min-time-capped group discussions and a missing human facilitator condition. There are also (mild) concerns of multiple testing issues, ie concerns that the study searched for effects in its analysis of the data. Further points of improvements include a more careful connection to the existing literature and a deeper engagement with socio-technical considerations.
I further note the disagreement among reviewers with regard to the relevance of the study for FAccT, which is scored and discussed differently.
Recommendation.
In my view, addressing specific concerns in a revision could generally improve the paper sufficiently, and I also agree with the rebuttal and the response by reviewer yCoR regarding the relevance of this work for FAccT. I would therefore propose the paper to be send to the revision track.
Requested revisions:
R1: Elaborate on the rational for 5-min discussion window, also as a limitation
R2: Report how the LLMs intervened during the discussions in more detail
R3: Improve the connection to prior related work
R4: Carefully engage with socio-technical considerations, including a prominent discussion of the missing human facilitator condition
Overall Recommendation: 2. Revise: The paper should be revised to address reviewers’ specific revision requests, and will be subject to re-review following the revision submission.


We thank all three reviewers for the thoughtful and detailed feedback. We appreciate the engagement with both the empirical design and the broader framing of the paper.
We are encouraged that two reviewers (R[cgHE], R[yCoR]) viewed the paper as a meaningful and timely contribution for FAccT, and appreciate R[YvfR]’s detailed critique. 
Our goal in revision is to (i) sharpen the paper’s FAccT positioning, (ii) better justify key design choices (especially the 5-minute window), (iii) improve transparency around facilitator interventions and analysis choices, and (iv) tighten scope/limitations to avoid overclaiming. Below, we first address shared concerns shared across reviewers, then respond to reviewer-specific points.
Shared concerns
1) Implementation details: five-minute discussion window, ceiling effects, and scope of claims (R[cgHE], R[yCoR])
The 5-minute discussion cap was chosen after multiple pilot rounds as a practical design tradeoff; for our within-participant design, each participant needed to complete all three treatment conditions within a one-hour session. 5-minutes per conversation (15 minutes total) satisfied this requirement, giving participants time to onboard, complete comprehension checks, complete allocation tasks and surveys, and wait for other participants given the synchronous task structure. While we mention this within the limitations, we will make this rationale explicit in the experimental design section. We can also report pilot data.
Furthermore, we will tighten claims in revision to clarify that our findings may be best interpreted in short-horizon, synchronous, low-to-moderate conflict group decision settings, rather than long-form or highly contentious deliberation.
We discuss ceiling effects and compare consensus metrics in the discussion, but we agree these points should be more prominent in the introduction and main results framing.
2) Consensus metrics and multi-dimensional evaluation framing (R[cgHE], R[yCoR])
We appreciate the concern that some conclusions could be read as relying too heavily on a narrow consensus metric. Our intent was to supplement the primary quantitative result (Krippendorff's alpha) with multi-dimensional evaluations (agreement, decision distributions, interaction dynamics, and participant perceptions).
We will revise the framing to make clearer that: i) the paper’s contribution is a multi-dimensional evaluation of LLM facilitation in group settings, ii) null effects on agreement should be interpreted in context (time window/task properties), and iii) meaningful shifts can occur in decision distributions and process dynamics even when agreement metrics do not move.
We will also make the discussion of the consensus metrics (including their behavior and limitations) more explicit in the main text.
3) Human facilitator baseline omission (R[yCoR], R[YvfR])
We agree that comparisons against a human baseline would provide a meaningful supplement to this work. We did not include a human facilitator condition primarily because recruiting, screening, training, and deploying human facilitators at the scale of our study (~100s of sessions) was prohibitively costly and operationally complex for this study design. In addition, a human-facilitator condition introduces substantial between-facilitator variance, which would require additional design/measurement choices to support clean comparison.
We acknowledge that the current draft does not explain this clearly enough. In revision, we will explicitly justify the omission in the design section and discuss the tradeoff more directly in limitations.
Response to R[YvfR]
Thank you for the detailed review and for recognizing the rigor of the experimental approach. We take your concerns seriously and believe several can be addressed through clearer framing and stronger signposting in revision. We address the human facilitator baseline omission in the shared responses above. Below we respond to your reviewer-specific concerns.
FAccT relevance. We respectfully disagree that this paper is primarily an IUI contribution rather than a FAccT one, and we believe this may reflect a framing mismatch in the current draft rather than a mismatch in contribution. In particular, the Experiences and Interactions track is relatively new, and we can make the paper’s connection to that track more explicit.
Our core contribution is an empirical study (N > 800) of AI-mediated group decision-making, examining how LLM facilitators affect collective outcomes, interaction dynamics, and participant perceptions of inclusion and helpfulness, in a consequential resource-allocation setting involving real charitable donations. We view this as directly relevant to FAccT’s newer Experiences and Interactions track, as the paper speaks to accountability in AI-mediated decisions and fairness in group interaction and participation.
We also note that this study depends on recent low-latency frontier models that make synchronous real-time facilitation feasible at scale, so this type of evaluation is newly feasible in practice. This is part of why we see the work as timely for FAccT’s evolving socio-technical scope, and we agree we should explain this more clearly in the introduction and related work.
We would also like to cite the view of the other two reviewers that this paper is a good fit for FAccT with R[yCoR] explicitly stating “I'd like to see this appear at FAccT as it makes a meaningful contribution to an important area.”
Literature positioning. We appreciate the request for stronger grounding and clearer differentiation from adjacent work. We can strengthen the paper’s positioning, especially relative to prior work focused on individual assistance, user satisfaction, or single-metric evaluation. We will also make the paper’s empirical gap clearer: real-time, synchronous, group decision-making with multi-dimensional evaluation of outcomes, process, and perceptions. Given R[cgHE]’s feedback that the work is “well situated within prior work on AI mediation, collective deliberation, and preference-based optimization,” we wonder if this concern is a framing/positioning issue that is addressable in revision rather than a fundamental weakness in the study itself.
Model selection rationale. We will expand the model-selection discussion to clarify the role of latency, cost, and accessibility constraints in a real-time synchronous setting, and why we benchmarked three comparable frontier models rather than aiming for exhaustive model coverage (including open-weight models). Our goal was to compare deployable, low-latency models under realistic interaction constraints, not to claim a comprehensive benchmark of all available model families.
Influence of LLM facilitators on group behavior/outcomes. While this analysis is present in the paper, it may not be sufficiently visible in the current framing. The paper directly analyzes how facilitation shapes allocations and interaction dynamics (Section 4.1 / Figure 5, plus discussion/conclusion). In revision, we will surface this earlier and connect it more explicitly to fairness/accountability concerns in AI-mediated group decisions.
We also appreciate the feedback on making the discussion’s practitioner-facing implications more explicit, and will revise section framing/titles to better surface what is substantively surprising and relevant.
We appreciate the push to strengthen the paper’s framing and positioning. We hope the clarifications above help resolve key points of disagreement, and we respectfully ask that you reconsider your assessment in light of this response and the planned revisions.
Response to R[yCoR]
Thank you for the thoughtful and balanced review. We appreciate your support for the paper’s relevance to FAccT and your framing of the work as a useful (and sobering) data point for collaborative AI. We address the shared concerns you raised (5-minute time limit/ceiling effects, consensus-metric framing, and human facilitator baseline omission) in responses above. Below we respond to your reviewer-specific points.
Abstraction / ecological validity. The study uses an intentionally controlled and abstracted task design. While this improves internal comparability, you’re right in that it limits direct real-world generalization. We will make this tradeoff more explicit earlier in the paper and tighten claims accordingly.
Perceived improvement vs. measured gains in group settings. We agree, this connection needs to be made more explicit. In revision, we will sharpen the discussion of why this divergence is especially salient in group settings, where AI can affect not only outcomes but also the social process (e.g., how discussion is structured, whose preferences are surfaced, and how compromise is framed).
Speed to outcome / productivity. We agree this is an important missing axis, particularly with respect to the adjacent literature on cognitive load. We will explicitly discuss this limitation and, if feasible within revision constraints, add a time/efficiency-related analysis using available platform logs/proxies.
Consensus metric interpretability. This is a good question. We will clarify the distinction between participant-facing task objectives/instructions (instruction figures in the appendix) and the measured consensus scores, and discuss whether that distinction limits participants’ ability to strategically optimize toward measured consensus. Given the ceiling effects observed in the data, we do not think that this would meaningfully affect results, but agree that this is an important detail to include.
Inclusion measure. We will clarify that our inclusion-related findings are based on participant perceptions (rather than a fully behavioral or externally validated inclusion measure), and tighten language accordingly.
Finally, we agree that some secondary results are too abstractly framed in the current draft. We will revise early framing sections (including the abstract/intro framing) to better map high-level constructs to concrete measures, surface key limitations earlier (including saturation risk), and better distinguish primary vs. exploratory analyses while clarifying the rationale for the reported metrics/tests.
Thank you again for the careful review. We appreciate the push to strengthen the paper’s framing and interpretation, and we will revise accordingly.
Response to R[cgHE]
Thank you for the careful and constructive review. We appreciate your positive assessment of the paper’s positioning, statistical transparency, and clarity, and we especially appreciate your concrete suggestions on improving our explanation of design decisions (e.g. facilitator intervention transparency).
We address the shared concerns you raised (5-minute discussion window/ceiling effects and consensus-metric framing) in the responses above. Below we respond to your reviewer-specific points.
Intervention timing/frequency and principles-guided triggers. We agree that the paper should more explicitly report when/how often the LLM intervened, and (for the principles-guided condition) how often specific failure modes were triggered. In revision, we will add clearer reporting of intervention timing/frequency across facilitation conditions, response latency (how quickly the LLM provided input), and failure-mode trigger frequencies in the principles-guided condition.
Representative transcript excerpts. We agree this would improve transparency and interpretability. We will include representative excerpts showing failure modes arising in context, the corresponding facilitator intervention, and the surrounding conversational dynamics within the 5-minute window.
Scope and interpretation of agreement-null results. We agree that the agreement-null result should be interpreted in light of task design constraints (including potential ceiling effects and the short discussion horizon). A clearer distinction between primary and secondary analyses may also help ground these results. In revision, we will tighten this framing and better emphasize the paper’s broader multi-dimensional contribution (including process, distribution, and perception effects).
Thank you again for the thoughtful review and actionable revision suggestions.




To the area chair and reviewers:

Thank you for the feedback and opportunity to revise our manuscript. We appreciate the reviewers’ careful reading and constructive feedback. 
Thank you for the thorough analysis. The following is a summary of the points we addressed in these revisions. All revisions appear as purple text throughout the manuscript - please pay attention to changes made in the Appendix as well, as we added several supplementary materials to address some specific concerns.
Shared concerns
1) Implementation details: five-minute discussion window, ceiling effects, and scope of claims (R[cgHE], R[yCoR])
We make this rationale explicit in the experimental design section, and also report pilot data, which was a key motivation for these changes.
Furthermore, we tightened claims in our revision to clarify that our findings may be best interpreted in short-horizon, synchronous, low-to-moderate conflict group decision settings, rather than long-form or highly contentious deliberation.
We make the ceiling effects and “selection” of consensus metrics more prominent in both the introduction and design / results sections. 
2) Consensus metrics and multi-dimensional evaluation framing (R[cgHE], R[yCoR])
We emphasize, in the introduction and experimental design, our intent to supplement the primary quantitative result (Krippendorff's alpha) with multi-dimensional evaluations (agreement, decision distributions, interaction dynamics, and participant perceptions).
We revised the framing to make clearer that: i) the paper’s contribution is a multi-dimensional evaluation of LLM facilitation in group settings, ii) null effects on agreement should be interpreted in context (time window/task properties), and iii) meaningful shifts can occur in decision distributions and process dynamics even when agreement metrics do not move.
We also discuss alternative consensus metrics, differences in outcome across methods, and why we settled on the Krippendorff alpha as the consensus metric focused on throughout this work. 
3) Human facilitator baseline omission (R[yCoR], R[YvfR])
In this revision, we explicitly justify the omission in the experiment design section and discuss the tradeoff more directly in limitations.
Response to R[YvfR]
FAccT relevance. We respectfully disagree that this paper is primarily an IUI contribution rather than a FAccT one, and we believe this may reflect a framing mismatch in the current draft rather than a mismatch in contribution. We rewrote our introduction, and several points of analysis, to explicitly highlight the relevance our paper has for FaccT’s Experiences and Interactions track.
Literature positioning. We strengthened the paper’s positioning, especially relative to prior work focused on individual assistance, user satisfaction, or single-metric evaluation. We also made the paper’s empirical gap clearer: real-time, synchronous, group decision-making with multi-dimensional evaluation of outcomes, process, and perceptions.
Model selection rationale. We expanded the model-selection discussion to clarify the role of latency, cost, and accessibility constraints in a real-time synchronous setting, and why we benchmarked three comparable frontier models rather than aiming for exhaustive model coverage (including open-weight models).
Influence of LLM facilitators on group behavior/outcomes. In revision, we surfaced discussions of the influence of LLM facilitators on group dynamics earlier and connected it more explicitly to fairness/accountability concerns in AI-mediated group decisions.

Response to R[yCoR]
Abstraction / ecological validity. The study uses an intentionally controlled and abstracted task design. While this improves internal comparability, you’re right in that it limits direct real-world generalization. We will make this tradeoff more explicit earlier in the paper and tighten claims accordingly.
Perceived improvement vs. measured gains in group settings. We agree, this connection needs to be made more explicit. In revision, we will sharpen the discussion of why this divergence is especially salient in group settings, where AI can affect not only outcomes but also the social process (e.g., how discussion is structured, whose preferences are surfaced, and how compromise is framed).
Speed to outcome / productivity. We agree this is an important missing axis, particularly with respect to the adjacent literature on cognitive load. We will explicitly discuss this limitation and, if feasible within revision constraints, add a time/efficiency-related analysis using available platform logs/proxies.
Consensus metric interpretability. This is a good question. We will clarify the distinction between participant-facing task objectives/instructions (instruction figures in the appendix) and the measured consensus scores, and discuss whether that distinction limits participants’ ability to strategically optimize toward measured consensus. Given the ceiling effects observed in the data, we do not think that this would meaningfully affect results, but agree that this is an important detail to include.
Inclusion measure. We will clarify that our inclusion-related findings are based on participant perceptions (rather than a fully behavioral or externally validated inclusion measure), and tighten language accordingly.
Finally, we agree that some secondary results are too abstractly framed in the current draft. We will revise early framing sections (including the abstract/intro framing) to better map high-level constructs to concrete measures, surface key limitations earlier (including saturation risk), and better distinguish primary vs. exploratory analyses while clarifying the rationale for the reported metrics/tests.
Thank you again for the careful review. We appreciate the push to strengthen the paper’s framing and interpretation, and we will revise accordingly.
Response to R[cgHE]
Thank you for the careful and constructive review. We appreciate your positive assessment of the paper’s positioning, statistical transparency, and clarity, and we especially appreciate your concrete suggestions on improving our explanation of design decisions (e.g. facilitator intervention transparency).
We address the shared concerns you raised (5-minute discussion window/ceiling effects and consensus-metric framing) in the responses above. Below we respond to your reviewer-specific points.
Intervention timing/frequency and principles-guided triggers. We agree that the paper should more explicitly report when/how often the LLM intervened, and (for the principles-guided condition) how often specific failure modes were triggered. In revision, we will add clearer reporting of intervention timing/frequency across facilitation conditions, response latency (how quickly the LLM provided input), and failure-mode trigger frequencies in the principles-guided condition.
Representative transcript excerpts. We agree this would improve transparency and interpretability. We will include representative excerpts showing failure modes arising in context, the corresponding facilitator intervention, and the surrounding conversational dynamics within the 5-minute window.
Scope and interpretation of agreement-null results. We agree that the agreement-null result should be interpreted in light of task design constraints (including potential ceiling effects and the short discussion horizon). A clearer distinction between primary and secondary analyses may also help ground these results. In revision, we will tighten this framing and better emphasize the paper’s broader multi-dimensional contribution (including process, distribution, and perception effects).
Thank you again for the thoughtful review and actionable revision suggestions.




Re: Area Chair:
However, there are also concerns regarding specific methodological choices. These include the 5-min-time-capped group discussions and a missing human facilitator condition. There are also (mild) concerns of multiple testing issues, ie concerns that the study searched for effects in its analysis of the data. Further points of improvements include a more careful connection to the existing literature and a deeper engagement with socio-technical considerations.
I further note the disagreement among reviewers with regard to the relevance of the study for FAccT, which is scored and discussed differently.
Recommendation.
In my view, addressing specific concerns in a revision could generally improve the paper sufficiently, and I also agree with the rebuttal and the response by reviewer yCoR regarding the relevance of this work for FAccT. I would therefore propose the paper to be send to the revision track.
Requested revisions:
R1: Elaborate on the rational for 5-min discussion window, also as a limitation
R2: Report how the LLMs intervened during the discussions in more detail
R3: Improve the connection to prior related work
R4: Carefully engage with socio-technical considerations, including a prominent discussion of the missing human facilitator condition
Overall Recommendation: 2. Revise: The paper should be revised to address reviewers’ specific revision requests, and will be subject to re-review following the revision submission.


We thank all three reviewers for the thoughtful and detailed feedback. We appreciate the engagement with both the empirical design and the broader framing of the paper.
We are encouraged that two reviewers (R[cgHE], R[yCoR]) viewed the paper as a meaningful and timely contribution for FAccT, and appreciate R[YvfR]’s detailed critique. 
Our goal in revision is to (i) sharpen the paper’s FAccT positioning, (ii) better justify key design choices (especially the 5-minute window), (iii) improve transparency around facilitator interventions and analysis choices, and (iv) tighten scope/limitations to avoid overclaiming. Below, we first address shared concerns shared across reviewers, then respond to reviewer-specific points.
Shared concerns
1) Implementation details: five-minute discussion window, ceiling effects, and scope of claims (R[cgHE], R[yCoR])
The 5-minute discussion cap was chosen after multiple pilot rounds as a practical design tradeoff; for our within-participant design, each participant needed to complete all three treatment conditions within a one-hour session. 5-minutes per conversation (15 minutes total) satisfied this requirement, giving participants time to onboard, complete comprehension checks, complete allocation tasks and surveys, and wait for other participants given the synchronous task structure. While we mention this within the limitations, we will make this rationale explicit in the experimental design section. We can also report pilot data.
Furthermore, we will tighten claims in revision to clarify that our findings may be best interpreted in short-horizon, synchronous, low-to-moderate conflict group decision settings, rather than long-form or highly contentious deliberation.
We discuss ceiling effects and compare consensus metrics in the discussion, but we agree these points should be more prominent in the introduction and main results framing.
2) Consensus metrics and multi-dimensional evaluation framing (R[cgHE], R[yCoR])
We appreciate the concern that some conclusions could be read as relying too heavily on a narrow consensus metric. Our intent was to supplement the primary quantitative result (Krippendorff's alpha) with multi-dimensional evaluations (agreement, decision distributions, interaction dynamics, and participant perceptions).
We will revise the framing to make clearer that: i) the paper’s contribution is a multi-dimensional evaluation of LLM facilitation in group settings, ii) null effects on agreement should be interpreted in context (time window/task properties), and iii) meaningful shifts can occur in decision distributions and process dynamics even when agreement metrics do not move.
We will also make the discussion of the consensus metrics (including their behavior and limitations) more explicit in the main text.
3) Human facilitator baseline omission (R[yCoR], R[YvfR])
We agree that comparisons against a human baseline would provide a meaningful supplement to this work. We did not include a human facilitator condition primarily because recruiting, screening, training, and deploying human facilitators at the scale of our study (~100s of sessions) was prohibitively costly and operationally complex for this study design. In addition, a human-facilitator condition introduces substantial between-facilitator variance, which would require additional design/measurement choices to support clean comparison.
We acknowledge that the current draft does not explain this clearly enough. In revision, we will explicitly justify the omission in the design section and discuss the tradeoff more directly in limitations.
Response to R[YvfR]
Thank you for the detailed review and for recognizing the rigor of the experimental approach. We take your concerns seriously and believe several can be addressed through clearer framing and stronger signposting in revision. We address the human facilitator baseline omission in the shared responses above. Below we respond to your reviewer-specific concerns.
FAccT relevance. We respectfully disagree that this paper is primarily an IUI contribution rather than a FAccT one, and we believe this may reflect a framing mismatch in the current draft rather than a mismatch in contribution. In particular, the Experiences and Interactions track is relatively new, and we can make the paper’s connection to that track more explicit.
Our core contribution is an empirical study (N > 800) of AI-mediated group decision-making, examining how LLM facilitators affect collective outcomes, interaction dynamics, and participant perceptions of inclusion and helpfulness, in a consequential resource-allocation setting involving real charitable donations. We view this as directly relevant to FAccT’s newer Experiences and Interactions track, as the paper speaks to accountability in AI-mediated decisions and fairness in group interaction and participation.
We also note that this study depends on recent low-latency frontier models that make synchronous real-time facilitation feasible at scale, so this type of evaluation is newly feasible in practice. This is part of why we see the work as timely for FAccT’s evolving socio-technical scope, and we agree we should explain this more clearly in the introduction and related work.
We would also like to cite the view of the other two reviewers that this paper is a good fit for FAccT with R[yCoR] explicitly stating “I'd like to see this appear at FAccT as it makes a meaningful contribution to an important area.”
Literature positioning. We appreciate the request for stronger grounding and clearer differentiation from adjacent work. We can strengthen the paper’s positioning, especially relative to prior work focused on individual assistance, user satisfaction, or single-metric evaluation. We will also make the paper’s empirical gap clearer: real-time, synchronous, group decision-making with multi-dimensional evaluation of outcomes, process, and perceptions. Given R[cgHE]’s feedback that the work is “well situated within prior work on AI mediation, collective deliberation, and preference-based optimization,” we wonder if this concern is a framing/positioning issue that is addressable in revision rather than a fundamental weakness in the study itself.
Model selection rationale. We will expand the model-selection discussion to clarify the role of latency, cost, and accessibility constraints in a real-time synchronous setting, and why we benchmarked three comparable frontier models rather than aiming for exhaustive model coverage (including open-weight models). Our goal was to compare deployable, low-latency models under realistic interaction constraints, not to claim a comprehensive benchmark of all available model families.
Influence of LLM facilitators on group behavior/outcomes. While this analysis is present in the paper, it may not be sufficiently visible in the current framing. The paper directly analyzes how facilitation shapes allocations and interaction dynamics (Section 4.1 / Figure 5, plus discussion/conclusion). In revision, we will surface this earlier and connect it more explicitly to fairness/accountability concerns in AI-mediated group decisions.
We also appreciate the feedback on making the discussion’s practitioner-facing implications more explicit, and will revise section framing/titles to better surface what is substantively surprising and relevant.
We appreciate the push to strengthen the paper’s framing and positioning. We hope the clarifications above help resolve key points of disagreement, and we respectfully ask that you reconsider your assessment in light of this response and the planned revisions.
Response to R[yCoR]
Thank you for the thoughtful and balanced review. We appreciate your support for the paper’s relevance to FAccT and your framing of the work as a useful (and sobering) data point for collaborative AI. We address the shared concerns you raised (5-minute time limit/ceiling effects, consensus-metric framing, and human facilitator baseline omission) in responses above. Below we respond to your reviewer-specific points.
Abstraction / ecological validity. The study uses an intentionally controlled and abstracted task design. While this improves internal comparability, you’re right in that it limits direct real-world generalization. We will make this tradeoff more explicit earlier in the paper and tighten claims accordingly.
Perceived improvement vs. measured gains in group settings. We agree, this connection needs to be made more explicit. In revision, we will sharpen the discussion of why this divergence is especially salient in group settings, where AI can affect not only outcomes but also the social process (e.g., how discussion is structured, whose preferences are surfaced, and how compromise is framed).
Speed to outcome / productivity. We agree this is an important missing axis, particularly with respect to the adjacent literature on cognitive load. We will explicitly discuss this limitation and, if feasible within revision constraints, add a time/efficiency-related analysis using available platform logs/proxies.
Consensus metric interpretability. This is a good question. We will clarify the distinction between participant-facing task objectives/instructions (instruction figures in the appendix) and the measured consensus scores, and discuss whether that distinction limits participants’ ability to strategically optimize toward measured consensus. Given the ceiling effects observed in the data, we do not think that this would meaningfully affect results, but agree that this is an important detail to include.
Inclusion measure. We will clarify that our inclusion-related findings are based on participant perceptions (rather than a fully behavioral or externally validated inclusion measure), and tighten language accordingly.
Finally, we agree that some secondary results are too abstractly framed in the current draft. We will revise early framing sections (including the abstract/intro framing) to better map high-level constructs to concrete measures, surface key limitations earlier (including saturation risk), and better distinguish primary vs. exploratory analyses while clarifying the rationale for the reported metrics/tests.
Thank you again for the careful review. We appreciate the push to strengthen the paper’s framing and interpretation, and we will revise accordingly.
Response to R[cgHE]
Thank you for the careful and constructive review. We appreciate your positive assessment of the paper’s positioning, statistical transparency, and clarity, and we especially appreciate your concrete suggestions on improving our explanation of design decisions (e.g. facilitator intervention transparency).
We address the shared concerns you raised (5-minute discussion window/ceiling effects and consensus-metric framing) in the responses above. Below we respond to your reviewer-specific points.
Intervention timing/frequency and principles-guided triggers. We agree that the paper should more explicitly report when/how often the LLM intervened, and (for the principles-guided condition) how often specific failure modes were triggered. In revision, we will add clearer reporting of intervention timing/frequency across facilitation conditions, response latency (how quickly the LLM provided input), and failure-mode trigger frequencies in the principles-guided condition.
Representative transcript excerpts. We agree this would improve transparency and interpretability. We will include representative excerpts showing failure modes arising in context, the corresponding facilitator intervention, and the surrounding conversational dynamics within the 5-minute window.
Scope and interpretation of agreement-null results. We agree that the agreement-null result should be interpreted in light of task design constraints (including potential ceiling effects and the short discussion horizon). A clearer distinction between primary and secondary analyses may also help ground these results. In revision, we will tighten this framing and better emphasize the paper’s broader multi-dimensional contribution (including process, distribution, and perception effects).
Thank you again for the thoughtful review and actionable revision suggestions.

Meta-review
 Metareview:
Submission summary.
The paper studies how LLM facilitators affect collective outcomes of group tasks. The paper draws on two experimental studies that vary the LLM facilitator model and strategy, and reports mixed findings with regards to the role of LLM facilitators, indicating steering effects regarding the allocation outcomes while consensus scores remain largely unaffected.
Discussion summary.
Three reviewers have evaluated the paper with mixed conclusions.
The reviews value the well-designed and well-powered experiments and the scope of the studied outcomes. The reviews also note the overall clarity of the paper and insights that are of relevance to the community.
However, there are also concerns regarding specific methodological choices. These include the 5-min-time-capped group discussions and a missing human facilitator condition. There are also (mild) concerns of multiple testing issues, ie concerns that the study searched for effects in its analysis of the data. Further points of improvements include a more careful connection to the existing literature and a deeper engagement with socio-technical considerations.
I further note the disagreement among reviewers with regard to the relevance of the study for FAccT, which is scored and discussed differently.
Recommendation.
In my view, addressing specific concerns in a revision could generally improve the paper sufficiently, and I also agree with the rebuttal and the response by reviewer yCoR regarding the relevance of this work for FAccT. I would therefore propose the paper to be send to the revision track.
Requested revisions:
R1: Elaborate on the rational for 5-min discussion window, also as a limitation
Section 3 (Experiment design): Added a paragraph explaining that the 5-minute limit was chosen based on N=20 pilots to ensure participants could complete the study within an hour and minimize fatigue, targeting "short-horizon, synchronous, and low-to-moderate disagreement group decision settings."
Section 4.3 (Interaction dynamics): Acknowledges that the 5-minute window likely impacted verbosity.
Section 6 (Limitations): Expands on the time limits, noting that some discussions ended artificially rather than reaching natural convergence.
Appendix G.2: Shows that despite the short window, the LLM detected and intervened on failure modes hundreds of times (e.g., 636 times for NoJustificationOrPrematureConsensus).
R2: Report how the LLMs intervened during the discussions in more detail
Section 4.3: Added a new paragraph "\rev{Facilitator Triggers and Latency}".
Appendix G.1: Added a massive section of full, representative chat transcripts showing exactly how the LLM summarized and intervened.
Appendix G.2: Added a detailed matrix (Table 12) showing exactly which failure modes triggered which LLM solutions.
R3: Improve the connection to prior related work
Section 1.1 (Related Work): Wove in several new citations. They explicitly call out limitations of prior work (e.g., cost/difficulty of scaling human participants) and frame how this paper addresses the gap. They added references to specific mediation strategies (CCE, TKI) and open character training (Maiya 2025; Papachristou 2025) to contextualize their principles-based prompt.
R4: Carefully engage with socio-technical considerations, including a prominent discussion of the missing human facilitator condition
Section 1 (Introduction): Rewrote the opening paragraph to explicitly state: "\rev{This new modality of human-AI interactions raises fairness and socio-technical concerns regarding the impact LLM systems are having on human and group dynamics.}"
Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Overall Recommendation: 2. Revise: The paper should be revised to address reviewers’ specific revision requests, and will be subject to re-review following the revision submission.

R1 
Summary Of Contribution:
This paper studies whether LLMs can improve group decision-making in short, real-time discussions over charitable allocations. Using large online experiments with over 800 participants, it finds that AI facilitators are popular and influence how money is divided, but do not meaningfully increase agreement among participants.
Quality:
The paper is well situated within prior work on AI mediation, collective deliberation, and preference-based optimization. It clearly distinguishes its multi-dimensional evaluation approach from earlier studies that focus only on satisfaction or agreement.
The main findings are supported by well-powered experiments, clear outcome measures, and transparent statistical analysis. Some conclusions about the lack of performance improvement rely heavily on a narrow consensus metric and a ceiling-prone task design (e.g., the task is low-conflict and short in duration, which limits coverage of settings where facilitation is most consequential).
	Section 3.5 (Incentives and payment): Added text clarifying that participants were not required to understand Krippendorff’s alpha. They only needed to pass a comprehension check understanding that "more agreement across participants translates to higher spending outcome."


Clarity:
The paper is clearly written, logically structured, and very easy to follow from motivation through results and discussion. Key concepts, conditions, and outcomes are consistently defined and revisited.
However, the choice of capping the discussion at five-minutes is not well justified. Were different study lenghts tested during the pilots? As reported in the paper, this time allowed only a handful of messages per participant and little time for disagreement or coordination problems to emerge. In facilitator conditions, the LLM intervenes roughly once per minute, reducing human back-and-forth and potentially shaping decisions before natural negotiation unfolds (see Fig. 2 and all 4 group members speaking almost at the same time). Since the principles-based facilitator is designed to act only when “failure modes” appear, it is unclear whether the time window is long enough for such failures to arise at all.
		Section 3 (Experiment design): Added a paragraph explaining that the 5-minute limit was chosen based on N=20 pilots to ensure participants could complete the study within an hour and minimize fatigue, targeting "short-horizon, synchronous, and low-to-moderate disagreement group decision settings."
Section 4.3 (Interaction dynamics): Acknowledges that the 5-minute window likely impacted verbosity.
Section 6 (Limitations): Expands on the time limits, noting that some discussions ended artificially rather than reaching natural convergence.
Appendix G.2: Shows that despite the short window, the LLM detected and intervened on failure modes hundreds of times (e.g., 636 times for NoJustificationOrPrematureConsensus).
Originality And Impact:
The paper clearly distinguishes itself from earlier studies that focus primarily on user satisfaction or single outcome measures by jointly analyzing agreement, decision distributions, interaction dynamics, and participant perceptions in real-time group settings. The research addresses a timely and important gap in understanding how LLMs function as actors in collective decision-making rather than as individual assistants.
Relevance To The Conference: 4. Agree that this submission is relevant to FAccT
Overall Recommendation: 4. A weak accept. I lean towards accepting this submission, but rejecting it would not be a serious issue.
Revision: Yes

R2
Summary Of Contribution:
Overall, this paper describes a study that was mostly well-executed and analyzed on an important topic for the FAccT community (AI-assisted consensus-making) and beyond (e.g. CSCW, HCI). The study is quite abstracted from the real world and the data is mined for signals that may or may not exist, so the work and paper definitely has its weaknesses. That said, I'd like to see this appear at FAccT as it makes a meaningful contribution to an important area.
Quality:
Strengths:
This was a bit of a sobering data point for anyone working in the collaborative AI space, and that's good! Another study that suggests (along with Alsobay et al., etc.) that there's no easy magic bullet here. I don't think anyone reading this paper could disagree that this is a data point we should pay attention to, even with its limitations.
The theme of differences with perceived improvement, but not actual productivity gains is something that resonated with me and perhaps is a theme the authors could unpack more in discussion / at the conference. It's a broad them across a lot (though certainly not all) AI experiences well beyond collaboration, e.g. AI Overviews. I didn't quite understand the argument about why this is particularly salient in group settings, however. The heterogeneous preferences component is definitely important, but the connection between these two needs to be strengthened. Is there some kind of lowest common denominator argument here? If so, let's articulate it explicitly and reflect on its strengths and weaknesses.
Weaknesses:
One major missing component of the analysis was speed to outcome
Section 6 (Limitations): Added a new paragraph "\rev{Speed to outcome}" explaining that because the timer was hard-capped at 5 minutes and automatically cut people off, it is difficult to reliably quantify if the LLM made them reach consensus faster.
. From a productivity standpoint, even if the outcomes are the same, if they were achieved with less cost (with speed being usually a key indicator of that), there are going to be productivity benefits. So, perhaps this study shows people still "agree to disagree", but get there faster? I'd like to see that at least mentioned in Discussion and/or Limitations if it isn't added to the paper.
Section 4.3: Added a new paragraph "\rev{Facilitator Triggers and Latency}".
Appendix G.1: Added a massive section of full, representative chat transcripts showing exactly how the LLM summarized and intervened.
Appendix G.2: Added a detailed matrix (Table 12) showing exactly which failure modes triggered which LLM solutions.
Section 6 (Limitations): Added a new paragraph "\rev{Speed to outcome}" explaining that because the timer was hard-capped at 5 minutes and automatically cut people off, it is difficult to reliably quantify if the LLM made them reach consensus faster.
Some of the limitations should be made clear earlier in the paper, e.g. the saturation risk.
Section 6 (Limitations): Expands on the time limits, noting that some discussions ended artificially rather than reaching natural convergence.
Section 6 (Limitations): Added a new paragraph "\rev{Speed to outcome}" explaining that because the timer was hard-capped at 5 minutes and automatically cut people off, it is difficult to reliably quantify if the LLM made them reach consensus faster.
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Were the metrics of consensus too hard for people to understand, which made it difficult for them to make decisions to drive it?
Section 3.5 (Incentives and payment): Added text clarifying that participants were not required to understand Krippendorff’s alpha. They only needed to pass a comprehension check understanding that "more agreement across participants translates to higher spending outcome."
There was no comparison to a human facilitator, which would have been useful for reference and from a "fairness is a process" standpoint. For instance, a human facilitator might in theory also change the distribution of charities? Would that affect the interpretation?
Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work.
The data re inclusion seemed weak; was it just perceived inclusion?
Section 5 (Discussion): Under "Perceived inclusion is not the same as participation equality", they added a sentence acknowledging this: "\rev{In future work, more concrete (less perception-based) measurements of inclusion should also be included to further quantify the impacts...}"
Much of the paper slices and dices the datasets in ways that may be statistically significant, but run into the classic risks of finding significance in this context.
Section 3.5 (Sample size rationale): Added a note that the study was strictly powered for the primary research questions (delta-consensus and preference). They state: "\rev{Subsequent analysis of steering effects and conversational dynamics were performed as a followup exploratory analysis. To avoid the risk associated with multiple statistical comparisons... we rely on the magnitude of effect sizes and the consistency of observed trends...}"
Clarity:
Some of the writing can be clarified: While the main results are clear, the secondary results are written in ways that hard to understand without an in-depth read of the paper (e.g. Section 1.2, abstract). Lots of high-level constructs are used that don't have an intuitive mapping and thus need to be explained.
Originality And Impact:
See above
Relevance To The Conference: 4. Agree that this submission is relevant to FAccT
Overall Recommendation: 4. A weak accept. I lean towards accepting this submission, but rejecting it would not be a serious issue.
Revision: No


R3
Summary Of Contribution:
This paper seeks answers to how groups of individuals can be facilitated by large language models in a discussion on allocating resources to myriad charities. The paper presents the findings of two empirical studies, where participants were grouped into a trio and asked to allocate a real donation budget across these charities, after a text-based discussion with the LLM facilitator. In the first study, the investigation varied the facilitating model between Gemini 2.5 Dash, Claude 4.5 Haiku, and GPT 5.1 Mini, seeking answers to which model participants reacted most positively to. In the second study, the investigation held the model fixed, and it instead varied the facilitation strategies between three treatments: summarization-style, principles-guided, and no-facilitation. Overall, the paper reports no significant differences when an LLM facilitator was introduced, yet participants' comments revealed that they reacted positively to the presence of the LLM facilitator, such as how it added structure or engaged participants in productive questioning.
Overall, I appreciated the rigorous approach applied to the experiments in this paper. However, I unfortunately could not recommend acceptance to FAccT. I make my recommendation for two reasons; first, I struggled with the alignment between the paper's topic and the FAccT call for submissions. One possible connection could be in the decision-support with human-in-the-loop space, but as stated, this paper reads more closely with an ACM IUI audience. When I think about a FAccT submission it's the exploration of fairness, accountability, and transparency that I focus on as my litmus test. This paper provides a thorough evaluation of an intelligent user interface, but I did not see a clear alignment to the particular topics in FAccT. Putting that aside, I also found several opportunities for improvement with this paper that I believe would place too much pressure on the authors to complete in the 2-3 week timeline for the revision cycle. I wanted to thank the authors for the opportunity to review their work, and I hope that my comments are helpful to them.
Quality:
Although I find this work to be generally good quality, and I enjoyed the rigorous approach towards the experiments in this study, I found some opportunities for improvement in the following areas:
The relevance to FAccT being made more explicit.
Section 1 (Introduction): Rewrote the opening paragraph to explicitly state: "\rev{This new modality of human-AI interactions raises fairness and socio-technical concerns regarding the impact LLM systems are having on human and group dynamics.}"
A stronger tie between this work and existing literature.
Section 1.1 (Related Work): Wove in several new citations. They explicitly call out limitations of prior work (e.g., cost/difficulty of scaling human participants) and frame their paper as addressing this gap. They added references to specific mediation strategies (CCE, TKI) and open character training (Maiya 2025; Papachristou 2025) to contextualize their principles-based prompt.
Socio-technical considerations that might explain the phenomena observed.
Relevance to FAccT
As I mentioned in my summary of contribution above, one of the primary areas that I could see an alignment between this paper and topics relevant to FAccT would be the decision-support with human-in-the-loop space. To deliver on this, one recommendation I would have would be to rework the introduction to make it very clear how this work ties in to topics relevant to FAccT. Is it that facilitation shows a level of bias when a human is involved? What kinds of bias are present that might be mitigated by LLMs? What kind of biases are potentially introduced by LLMs as facilitators? These would be some motivations to make a clearer connection with FAccT (as opposed to IUI).
Section 1 (Introduction): Rewrote the opening paragraph to explicitly state: "\rev{This new modality of human-AI interactions raises fairness and socio-technical concerns regarding the impact LLM systems are having on human and group dynamics.}"
Connection to prior literature
This portion is a recurring theme for my review, because I do not believe that the engagement with the prior literature is sufficient to solidify for reviewers how this paper fits into the broader landscape of the literature. Overall, I believe that the paper needs to make more concrete connections between itself and the existing literature. One technique that I have seen that makes these concrete ties are statements such as "although Authors et al. investigated phenomenon X, this paper differs from Authors et al. by instead investigating phenomenon Y" at the end of paragraphs. This would help to connect what gaps in the research landscape this paper fills, providing reviewers the ability to situate it in the context of the literature.
Socio-technical considerations
This, for me, was one of the areas that the paper did not explore in sufficient depth, and it unfortunately introduced a somewhat large blind spot in the experimental design. Facilitation has been used in legal contexts to resolve disputes, but this paper makes an implicit assumption that having an intelligent system as a facilitator is "the" solution. On its face, introducing a "no facilitation" baseline seems to address this, but it can't reasonably be compared against other socio-technical considerations like "what if there was a human facilitator?" 
Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Specifically, the comparison is set up that "some AI is better than no AI", which points to the technical consideration. However, as social creatures, what would have happened if the study had had a human facilitator in the session, guiding the trio?
Clarity:
I found that this work was generally clearly written and self-contained, and the methodology was generally well-conveyed to give reviewers a sense for participants' tasks. However, I found some opportunities for improvement in the following areas:
Greater communication on the model selection.
Introduction: Points to a new appendix.
Appendix F.2 (Model selection and parameters): Added an explanation that they chose the SOTA low-latency, closed-source models. They explicitly mention that an open-source model (like LLaMa) was excluded to avoid sample size explosion and because open-source models currently require massive infrastructure investments to match the conversational latency of frontier APIs.
Greater transparency for why a "human facilitator" condition was not also included as an experimental baseline.
Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Model Selection
The paper is very transparent about the three models it selected, but I wanted some additional information about why those particular models were selected. Did an engineering choice of platform limit the models selected? What considerations were factored in to selecting these three models? Notably, LLaMa is missing from this set, although it has literary evidence suggesting its capabilities on adopting different personas and how it communicates to others (e.g., [1,2]). I would have liked to see a more detailed discussion regarding model selection to help me understand why these particular models were expected to behave the "best" for whatever metric was being optimized.
	Introduction: Points to a new appendix.
Appendix F.2 (Model selection and parameters): Added an explanation that they chose the SOTA low-latency, closed-source models. They explicitly mention that an open-source model (like LLaMa) was excluded to avoid sample size explosion and because open-source models currently require massive infrastructure investments to match the conversational latency of frontier APIs.


Human-Facilitator Condition
See my "socio-technical considerations" portion above for more details. I would have liked to see more discussion on whether and how this condition was considered and subsequently dropped.
References
[1] Maiya, S., Bartsch, H., Lambert, N., & Hubinger, E. (2025). Open character training: Shaping the persona of AI assistants through constitutional AI. arXiv preprint arXiv:2511.01689. [2] Thakur, H., Agrawal, E., & Mukund, S. (2025). Personas within parameters: Fine-tuning small language models with low-rank adapters to mimic user behaviors. arXiv preprint arXiv:2509.09689.
	Section 3.3: Added a robust paragraph explaining why human facilitators were excluded: prohibitive operational/scaling costs, and the massive statistical variance introduced by a pool of human mediators (which would muddy the data regarding LLM specific dynamics).
Section 6 (Limitations): Added a "\rev{Lack of human facilitators}" section explicitly calling this out for future work
Section 1.1 (Related Work): Wove in several new citations. They explicitly call out limitations of prior work (e.g., cost/difficulty of scaling human participants) and frame their paper as addressing this gap. They added references to specific mediation strategies (CCE, TKI) and open character training (Maiya 2025; Papachristou 2025) to contextualize their principles-based prompt.



Originality And Impact:
Regarding originality, this was one area that I believed was not clear enough to me that I highlighted in the Quality section above; overall, I believe that the paper needs to make more concrete connections between itself and the existing literature. In particular to this paper, I got the sense that perhaps summarization-style and principles-guided facilitation were not novel techniques? If I am correct in that assumption, then I would have liked to see more details in the Facilitator strategies and structured facilitation paragraph in 1.1 that discusses key findings from relevant works. This would provide additional context for reviewers to understand whether we should expect similar findings or not. If my assumption is incorrect, then a statement like "This paper is the first of its kind to investigate summarization-style and principles-guided facilitation in LLM facilitation" provides compelling evidence to support originality of the work.
Unfortunately, for impact, this also ties back to the connection between this work and prior literature. Without a more thorough exploration of the landscape formed from the prior literature, it becomes very difficult to assess potential gaps in the research landscape and the significance of the results. Additionally, the discussion section of the paper, which I have seen as the important section to provide implications for design or implications for practitioners, did not seem to deliver as powerful a message for practitioners, because the paragraph titles did not convey a message of why we should be surprised. For instance "People can prefer facilitation, even when it does not improve outcomes", "Facilitators can still shift what groups decide" and "preference depends on context", on their faces, do not help me as a practitioner understand why I should be surprised. The preference of facilitation has been used in legal context to resolve disputes between parties, even when these disputes are contentious. Facilitators can shift decisions can be seen as "over-reliance" on perceived expertise. I would have liked to see more engagement with prior literature that points to the opposite effect or empirical evidence that conveys why we, as practitioners, should have expected a different outcome.
Relevance To The Conference: 2. Disagree that this submission is relevant to FAccT
Overall Recommendation: 1. A strong reject. Paper is fundamentally flawed (e.g., major results are trivial, wrong, or already known). I strongly believe this submission should be rejected.
Revision: No



Flagged as MIssing by Gemini:
[7] The theme of differences with perceived improvement... unpack more in discussion (lowest common denominator / AI Overviews).
MISSING: The reviewer asked for you to explicitly articulate a "lowest common denominator argument" regarding heterogeneous preferences, and potentially compare the perception vs. productivity gap to broader AI features like "AI Overviews." This specific thematic expansion has not been added to the Discussion section.
[5] Originality / Framing of Discussion ("Why should we be surprised?").
MISSING / PARTIALLY ADDRESSED: While you integrated the reviewer's requested citations to establish originality in Section 1.1, you did not meaningfully alter the Section 5 (Discussion) framing. The reviewer specifically requested that you frame your Discussion paragraphs to tell practitioners why these results are surprising (e.g., framing the fact that facilitators shift decisions as a form of "over-reliance on perceived expertise" contrary to established legal/mediation literature). Updating the prose in the Discussion to reflect this "surprising" angle would fully satisfy this reviewer.
[4] Clarify how "fast" the LLM provided the input.
Addressed / Partially Addressed: In Section 3.3, text was added specifying the use of "state-of-the-art, low-latency frontier model variations to support affordable real-time interaction." Appendix F also notes that "thinking modes" were disabled to prevent latency. (Note: You do not provide exact millisecond latency times, but the conceptual concern regarding real-time flow is addressed).





==> representative_transcripts.tex <==
1. Study 2 - No facilitator, no consensus reached (5-min timeout, 33.3 consensus score alpha)

Zebra09:35:22.000
Hello! I think donating to clean ocean action is the most important out of the three
Zebra09:35:45.000
what does everyone else think?
Bear 209:36:50.000
I would give the most to global fund for women as this charity concerns people and rest are about nature
Buffalo09:36:51.000
I do think that cleaning the oceans is the most urgent and impactful of the three.
Zebra09:37:10.000
why do you think it's not important?
Zebra09:37:26.000
sorry I meant important
Buffalo09:37:36.000
Helping woman is more important than helping animals so I support it.
Zebra09:38:13.000
I think if we don't support nature it will have a negative affect on humans therefore I think it's the most importan
Buffalo09:38:45.000
I would rank cleaning the oceans and helping women as the two most urgent with helping animals as third.
Zebra09:39:14.000
So should we put cleaning the oceans as most important?
Bear 209:39:29.000
I would put the women as more important
Bear 209:39:43.000
but let's allocate like 30% toward oceans
Zebra09:40:09.000
what are your arguments for allocating so much towards women?


2. Study 2 - No facilitator, consensus reached (alpha = 100)
Lion11:29:02.000
Hello
Bear11:29:05.000
hello
Cat11:29:08.000
Hi
Lion11:29:23.000
So how should we allocate the donations?
Cat11:29:34.000
I think aids 4 children should get 50%
Bear11:29:45.000
ill be honest i just split it 50/50 between the water aid and village children
Cat11:30:00.000
30% 4 global fund for women
Cat11:30:23.000
Water aid comes last for me
Lion11:30:28.000
Ok so Bear it's 25% for water and 25% for children?
Bear11:30:56.000
nah as in 50% each one
Cat11:31:11.000
Bear we have 3 charities
Bear11:31:14.000
the women one is too vague for me
Lion11:31:19.000
So you don't want to allocate any donations for women then?
Lion11:31:28.000
I guess that's an option too
Cat11:31:43.000
I think we should allocate for all
Bear11:31:43.000
i know but whats the money actually getting used for exactly is my only concern
Lion11:32:05.000
Hmm
Bear11:32:25.000
allocating some is fine i jusy think the other two are a bigger a priotity
Lion11:32:28.000
I went 20% for women
Cat11:32:38.000
yes the cause is briliant and global with the children
Lion11:32:40.000
50% for children 30% for ocean
Bear11:32:54.000
yeah thats fine
Cat11:32:56.000
I can agree with Lion
Bear11:33:03.000
sounds good
Cat11:33:21.000
50% for children 30% for ocean and 20% for women
Lion11:33:33.000
ok
Cat11:33:36.000
ok
Bear11:33:39.000
cool
System11:34:07.000
The timer for this stage has ended; you can no longer respond.
System11:34:07.000
The timer for this stage has ended; you can no longer respond.
System11:34:10.000
Bear has left the chat.
System11:34:12.000
Lion has left the chat.
System11:34:20.000
Cat has left the chat.


3. Study 1 - Claude Facilitator

Facilitator16:44:12.000
Welcome to Round 2! �� We're here to discuss how to allocate donations across three important causes:�� **Global Housing for Orphans** - providing shelter and homes for vulnerable children�� **Clean Ocean Action** - protecting marine ecosystems and addressing ocean pollution�� **International Fund for Animal Welfare (IFAW)** - supporting wildlife conservation and animal protectionI'd like to hear your thoughts on how we should split the donation. What matters most to each of you? What are your initial instincts on how to allocate these funds? Feel free to share your perspectives and we'll work together toward a consensus allocation.
Elephant16:44:53.000
I chose global at 70% is it okay guys?
Gorilla16:45:05.000
- Global Housing for Orphans receives the highest allocation (40%) because providing stable nurturing environments for orphans addresses immediate and critical needs for vulnerable children potentially impacting their entire lives. The combination of housing and education suggests a holistic approach to supporting their development.- Clean Ocean Action and IFAW both have very high Charity Navigator scores indicating strong effectiveness and transparency. I've allocated 30% to each to balance the critical environmental impact of ocean pollution with the important work of animal welfare and conservation that IFAW does. Both causes are significant for long-term ecological and animal well-being.
Gorilla16:45:24.000
Guy how about this
Tiger16:45:45.000
Gorilla l stay with you...
Elephant16:45:55.000
We put Global at 40%?
Facilitator16:46:00.000
Great discussion everyone! �� I'm seeing some nice convergence here. Let me recap where we're at:**Gorilla's proposal: 40% / 30% / 30%**- �� Global Housing for Orphans: 40% (addresses immediate critical needs for vulnerable children)- �� Clean Ocean Action: 30% (strong environmental impact)- �� IFAW: 30% (important wildlife conservation work)**Elephant** it sounds like you're moving from your initial 70% suggestion toward this more balanced split—is that right? **Tiger** you mentioned staying with Gorilla—does this allocation feel right to you as well?This approach balances immediate human welfare (housing for orphans) with long-term environmental and animal welfare impact. Before we finalize does everyone feel this represents a fair allocation of these three important causes? Any final thoughts or adjustments?
Tiger16:46:27.000
Yes
Elephant16:46:54.000
Lol yes
Facilitator16:46:58.000
Perfect! �� We've reached a strong group consensus! Here's our final allocation:**Final Donation Split:**- �� **Global Housing for Orphans: 40%**- �� **Clean Ocean Action: 30%**- �� **IFAW: 30%**This balanced approach addresses immediate human needs through housing for vulnerable children while ensuring meaningful support for critical environmental and animal welfare causes. Great collaborative discussion everyone! This allocation reflects both compassion for human welfare and commitment to long-term ecological and animal conservation. ✨
Elephant16:47:14.000
okay the 40 30 30 it is then
Gorilla16:47:30.000
That's great
Tiger16:47:35.000
40 3030. I think is fine
Elephant16:47:42.000
cool

4. Study 1 - GPT faciltiator
Butterfly16:47:22.000
hi
Facilitator16:47:28.000
Hi all — quick facilitation to get us moving. Goal: decide one exact allocation (percentages summing to 100) across the three charities: Rainforest Action (��) Aid for Children in Remote Villages (��) Sudan Humanitarian Aid (��).Please each do two short things in one reply: 1) name your top priority in one sentence and 2) propose an exact allocation (three integers that add to 100) e.g. 20/30/50 for ��/��/��.To seed the discussion here are three reasonable starting options you can pick or modify:- Option A (equal): 33/33/34 — treats all causes equally.- Option B (urgent need): 20/30/50 — prioritizes urgent humanitarian aid in Sudan.- Option C (prevention & long-term): 40/40/20 — prioritizes rainforest and children (longer-term impact).After everyone posts we’ll compute a combined proposal (e.g. average) and iterate until we reach consensus. Please reply with your priority + your proposed split now.
Llama16:47:29.000
hi
Swan16:47:30.000
hey budies
Facilitator16:47:40.000
Quick nudge: we still need each person's two short things so we can compute a combined proposal. Please in one reply do both: (1) state your top priority in one sentence and (2) give an exact allocation as three integers that add to 100 in the order Rainforest Action (��) / Aid for Children (��) / Sudan Humanitarian Aid (��). You can pick or tweak one of these seeds if helpful:- Option A (equal): 33/33/34- Option B (urgent need): 20/30/50- Option C (prevention & long-term): 40/40/20After all three of you post I will compute the combined (average) split and propose the next iterate. Please keep answers short.
Llama16:48:32.000
option b
Butterfly16:48:38.000
i think the last 2 choices should be our focus guys
Swan16:48:40.000
my was 40 for children 40 for sudan aid and 20 for rainforest
Facilitator16:49:00.000
Thanks — Llama gave 20/30/50 and Swan gave 20/40/40. Butterfly you didn’t provide exact integers yet: please post three integers that add to 100 in the order ��/��/��. Provisional combined average of Llama+Swan = 20/35/45 (Rainforest/Aid for Children/Sudan). Do you all accept 20/35/45 or propose a quick adjustment? Reply with 'accept' or your new 3-number split.
Llama16:49:18.000
accept
Swan16:49:18.000
option c
Butterfly16:49:24.000
my was 70 for sudan and 30 for children
Facilitator16:49:35.000
Quick check: Llama accepted 20/35/45; Swan said 'option c' (please confirm you mean 40/40/20 in the order ��/��/��). Butterfly you wrote 70 for Sudan and 30 for children — please give three integers that add to 100 in this exact order: Rainforest Action (��) / Aid for Children (��) / Sudan Humanitarian Aid (��). Once all three of you post explicit 3-number splits I will compute the combined (average) proposal and suggest the next iterate. Keep it short (one line).
Butterfly16:50:32.000
my allocation is 0/30/70
Swan16:50:35.000
humanitarian aid I think is most important than rainforest
Facilitator16:50:49.000
Combined (rounded) average proposal: 13/35/52 (�� / �� / ��). Calculations: Rainforest (20+20+0)/3 ≈13.3→13 Children (35+40+30)/3=35 Sudan (45+40+70)/3≈51.7→52. Please reply with 'accept' or give a new 3-number split (��/��/��). If you want suggest small tweaks (±5) rather than large changes so we can converge quickly.
Llama16:50:53.000
50/25/25
Facilitator16:51:07.000
New combined (rounded) average: 23/32/45 (��/��/��) based on Llama 50/25/25 Swan 20/40/40 Butterfly 0/30/70. Please reply with 'accept' or a small tweak (±5 on any category) and a new 3-number split so we can converge quickly. If you want in one sentence say why you prefer shifting funds.
Llama16:51:23.000
accept
Swan16:51:32.000
go 40-40-20
Swan16:51:47.000
20 for rainforest
Facilitator16:52:18.000
Combined proposal: 21/34/45 (�� / �� / ��). Calculation: (23+40+0)/3=21 (32+40+30)/3=34 (45+20+70)/3=45. Please reply 'accept' or give a small tweak (±5) as three integers summing to 100.
System16:52:22.000
The timer for this stage has ended; you can no longer respond.
System16:52:28.000
Butterfly has left the chat.
System16:52:31.000
Llama has left the chat.
System16:52:31.000
Swan has left the chat.

5. Study 1 - Gemini facilitator
Facilitator16:13:06.000
Hello everyone! Welcome to the discussion. Our goal for this round is to decide how to allocate a donation across three very worthy charities: �� WildAid �� International Fund for Animal Welfare (IFAW) and �� Global Housing for Orphans. We need to come to a group consensus on an exact percentage split for example 30%/40%/30%.To begin what are your initial thoughts or preferences on how we might distribute the funds? Please feel free to share your reasoning behind your suggestions!
Badger16:13:19.000
hi
Bear16:13:45.000
I chose the two animal charities to get 40 and the other at 20. Just because i am more an animal person than a kid person
Facilitator16:13:52.000
Thanks Bear for sharing your initial thoughts and your reasoning behind prioritizing the animal charities. That gives us a good starting point.Alligator and Badger what are your initial preferences regarding the allocation? Do you lean towards supporting certain causes more than others and what's your reasoning? Feel free to react to Bear's suggestion too if you have thoughts on it.
Badger16:14:11.000
i think animals have less welfare and fundraiser programs so i allocated for animal welfare than orphans
Badger16:14:17.000
*more
Alligator16:14:20.000
I went 50 50 on both animal ones because I like animals more then orphans lol but I can definitely change
Facilitator16:14:28.000
It's clear there's a strong preference within the group to prioritize the animal welfare charities WildAid and IFAW. Bear suggested a 40%/40%/20% split while Alligator leaned towards 50%/50% for the animal charities potentially leaving Global Housing for Orphans with 0%. Badger also expressed a strong preference for animal welfare. Given this shared sentiment how do we want to specifically differentiate between WildAid and IFAW? And is there any room or reasoning to allocate a portion to Global Housing for Orphans or are we firm on focusing solely on animal welfare? Let's try to refine these initial thoughts into a specific percentage proposal for all three.
Bear16:14:37.000
i could up both animal ones to 50 and be ok too
Badger16:15:05.000
there are so many organizations helping orphans.
Facilitator16:15:17.000
Thank you Bear and Badger for clarifying your leanings. It's very clear there's a strong preference to dedicate the funds primarily if not entirely to the animal welfare charities. Bear your suggestion of 50%/50% for WildAid and IFAW potentially leaving Global Housing for Orphans at 0% reflects this. Badger your point about other organizations focusing on orphans reinforces this perspective.So would the group be comfortable with a proposed split of 50% for �� WildAid 50% for �� International Fund for Animal Welfare (IFAW) and 0% for �� Global Housing for Orphans? Or given our goal is to allocate across all three would anyone like to make a case for a smaller symbolic percentage (e.g. 5-10%) for Global Housing for Orphans and how would that adjust the animal charity percentages?
Bear16:15:24.000
i would be ok with that
Facilitator16:15:32.000
Thanks Bear for confirming you're okay with the 50%/50%/0% split. Alligator and Badger what are your thoughts on this proposed distribution? Are you both comfortable with 50% to WildAid 50% to IFAW and 0% to Global Housing for Orphans or do you have any final adjustments or considerations you'd like to share?
Badger16:15:37.000
i'm okay with that too
Facilitator16:15:43.000
Thank you Bear and Badger for confirming your comfort with the 50%/50%/0% split. Alligator what are your thoughts? Are you also comfortable with a distribution of 50% for �� WildAid 50% for �� International Fund for Animal Welfare (IFAW) and 0% for �� Global Housing for Orphans? Once Alligator confirms we will have a clear group consensus on the allocation.
Alligator16:15:48.000
That sounds good to me
Facilitator16:15:54.000
Excellent! It's clear we have reached a unanimous consensus. Bear Badger and Alligator you've all confirmed your comfort with the proposed distribution. Therefore the group's final decision for the allocation is: * **�� WildAid: 50%*** **�� International Fund for Animal Welfare (IFAW): 50%*** **�� Global Housing for Orphans: 0%**Thank you all for your active participation and for coming to a clear resolution!
Badger16:16:31.000
imf also helps orphans and the government contributes a lot to child services
Badger16:16:49.000
animals get shit lol
Alligator16:17:00.000
That was my thinking too
Bear16:17:04.000
i like that we all picked animals!
Alligator16:17:43.000
Well that was easy lol
Bear16:17:58.000
proud of us haha
System16:18:07.000
The timer for this stage has ended; you can no longer respond.
Badger16:18:09.000
easy coffee and beer money
System16:18:13.000
Bear has left the chat.


STudy 2 - Principles-based mediator
Pig 310:31:11.000
hey guys whats your allocation
Gorilla 310:31:17.000
Hey guys I allocated 60 to woman and 20 to clean ocean and 20 to rainforest
Bear 310:32:33.000
i went 45% on woman 30% on the ocean and 25% on the forest nut felt likei should change the forest allocation as they are also equally important
Pig 310:32:41.000
40% FOR Women 30% to rainforest and 30% to clean ocean
Facilitator10:32:49.000
Thanks for sharing your initial allocations. What's one thing that influenced your own split or what do you notice about the allocations others have put forward?
Bear 310:33:27.000
the importance of each organization globally
Gorilla 310:33:43.000
true
Facilitator10:33:55.000
It sounds like global importance is on your minds. Considering the different allocations shared does anyone want to respond to or build on an allocation idea from someone else?
Bear 310:35:12.000
we could go equally but prioritize women and the forest
Facilitator10:35:35.000
Bear that's an interesting principle. How do others feel about this idea of 'equally but prioritizing women and the forest' especially as we work toward specific percentages across all three?
Gorilla 310:35:50.000
I think woman should be top priority
Pig 310:36:08.000
i think so too
System10:36:12.000
The timer for this stage has ended; you can no longer respond.
System10:36:19.000
Bear 3 has left the chat.
System10:36:27.000
Gorilla 3 has left the chat.
System10:37:04.000
Pig 3 has left the chat.


Study 2 - Summarization based
Facilitator11:42:11.000
Welcome everyone! Let's begin discussing the ideal allocation of donations across Global Housing for Orphans Clean Ocean Action and Rainforest Action. What are your initial thoughts on how we might split the funds?
Bear11:42:32.000
50% on oceans 25 for orphans and 25 for rainforest
Dolphin11:43:11.000
I did 40% rainforest 30% orphans and oceans. I'm not particularly learning towards any of the 3 since I think all are pretty important. So a little undecided I guess
Badger11:43:16.000
45% to housing for orphans25% for clean ocean and 30% for rainforest
Facilitator11:43:26.000
Thank you all for sharing your initial ideas. We have proposals prioritizing Clean Ocean Action (Bear) Rainforest Action (Dolphin) and Global Housing for Orphans (Badger). What are some of the key factors or reasons influencing your initial splits?
Badger11:43:49.000
l would prioritize human beings than anything else
Bear11:44:10.000
unedrstandable however oceans are very important for huamn beings too
Dolphin11:44:29.000
I allocated a little more for rainforest since there's much less of the rainforest left than ocean (i think). The other two I think are equally important
Badger11:44:31.000
how are oceans important to human beings
Facilitator11:44:39.000
It seems we're discussing different priorities here: direct human welfare broader environmental impact on human well-being and the urgency of disappearing resources. Understanding these different influences is key. What are your thoughts on comparing these types of impacts?
Bear11:44:49.000
Rainforests... I have some expireince with rainforests charities back in uni and they were not very good.
Bear11:45:23.000
Oceans are important for oxygen production from algae fish production water availability climate local weather
Facilitator11:45:29.000
It sounds like we're weighing a few different aspects now: direct human impact urgent environmental conservation broader long-term environmental benefits for humans and even considerations around the effectiveness or track record of different charities. How do these various factors align or conflict for you?
Dolphin11:45:48.000
yeah i did look at the description for the rainforest charity and it seems more focused on campaigning
Badger11:46:36.000
yes l agree the environment is also very importand
Dolphin11:46:45.000
I don't mind increasing my allocation for ocean since they mention plastic removal from oceans
Dolphin11:46:51.000
so a bit more specific
Badger11:46:55.000
so how should we alloctae
Bear11:46:57.000
Yeah oceans are doing some real job. Especially cleaning oceans from palstic so how about 45 for oceans 25 for forest
Bear11:47:02.000
30 for orphans\
Dolphin11:47:08.000
sounds good
System11:47:11.000
The timer for this stage has ended; you can no longer respond.
System11:47:17.000
Bear has left the chat.
System11:47:22.000
Badger has left the chat.
System11:47:27.000
Dolphin has left the chat.
Facilitator11:47:39.000
It sounds like Bear has proposed a new allocation of 45% for Clean Ocean Action 30% for Global Housing for Orphans and 25% for Rainforest Action. Dolphin has indicated agreement with this. Badger what are your thoughts on this updated proposal?
